Extreme Point Supervised Instance Segmentation

This paper introduces a novel approach to learning instance segmentation using extreme points, i.e., the topmost, leftmost, bottommost, and rightmost points, of each object. These points are readily available in the modern bounding box annotation process while offering strong clues for precise segmentation, and thus allows to improve performance at the same annotation cost with box-supervised methods. Our work considers extreme points as a part of the true instance mask and propagates them to identify potential foreground and background points, which are all together used for training a pseudo label generator. Then pseudo labels given by the generator are in turn used for supervised learning of our final model. On three public benchmarks, our method significantly outperforms existing box-supervised methods, further narrowing the gap with its fully supervised counterpart. In particular, our model generates high-quality masks when a target object is separated into multiple parts, where previous box-supervised methods often fail.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> sections/00_abstract_backup_0325.tex <==
\begin{abstract}
This paper introduces a new weakly supervised learning approach for instance segmentation using extreme points, \ie, the topmost, leftmost, bottommost, and rightmost points of an object.
Although these points are readily available in the 
 modern bounding box annotation process and offer strong clues for precise segmentation, they have received less attention in the literature.
Motivated by this, our study explores extreme point supervised instance segmentation to further enhance performance at the same annotation cost with box-supervised methods.
Our work considers extreme points as a part of the true instance mask and propagates them to identify potential foreground and background points, which are all together used for training a pseudo label generator.
Then pseudo labels given by the generator are in turn used for supervised learning of our final model.
Our model generates high-quality masks, particularly when the target object is separated into multiple parts, where previous box-supervised methods often fail.
On three public benchmarks, our method significantly outperforms existing box-supervised methods, further narrowing the gap with its fully supervised counterpart.


% This paper introduces a new weakly supervised learning approach for instance segmentation using extreme points, \ie, the topmost, leftmost, bottommost, and rightmost points of an object.
% Although these points are readily available during the bounding box annotation process and offer valuable clues for precise segmentation, they have received less attention in weakly supervised instance segmentation literature.
% Motivated by this, our study explores extreme point supervised instance segmentation to further enhance performance without increasing annotation costs compared to box-supervised methods.
% Our framework utilizes extreme points as a part of the true instance mask and exploits them as supervision for training a pseudo label generator.
% To train the generator, potential foreground and background points are estimated by propagating the extreme points.
% Pseudo segmentation labels from the generator are in turn used for supervised learning.
% Our method generates high-quality masks, particularly when the target object is separated into multiple parts, where previous box-supervised methods often fail.
% On three public benchmarks, our method significantly outperforms existing state-of-the-art methods in box-supervised instance segmentation, further narrowing the gap with its fully supervised counterpart.
\end{abstract}

==> sections/01_intro_backup_1116.tex <==
\section{Introduction}

%문단 구조 나누기. 핵심 내용 적기.
%1. instance segmentation 모델에 대한 설명. + instance segmentation task의 중요성 + weak sup 방식들이 나오게 된 이유.
%This technique is particularly invaluable in domains such as autonomous driving, robotic manipulation, and medical image analysis, where identifying specific entities like people, vehicles, and tumors is crucial.
Instance segmentation, a foundational task in computer vision, has made significant strides through supervised learning of deep neural networks ~\cite{mask_rcnn, wang2020solo, wang2020solov2, tian2020conditional, cheng2022masked}. 
However, its broader application is hindered since the required pixel-level masks are prohibitively expensive to obtain. \LHJmodified{thereby driving the pursuit of the weakly supervised approach. reference with other researhces like point scribble}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/Teaser_8.png}
    \end{subfigure}
    \caption{\textbf{Types of weak supervision for instance segmentation and their corresponding generated pseudo labels.} Top: A box-supervised method~\cite{Lan_2023_CVPR} struggles to generate an accurate pseudo label for the separated object. Bottom: Our approach leverages extreme points as weak supervision, attainable during the box annotation process at no extra cost, and generates a precise pseudo label for the separated object. Best viewed in color.}
    \label{fig:teaser}
    \vspace{-3mm}
\end{figure}

%2문단, box-supervised model에 대한 설명. 

Building on this momentum, research about box-supervised instance segmentation has gained considerable traction~\cite{khoreva2017simple, lee2021bbam, hsu2019weakly, tian2021boxinst, lan2021discobox, li2022box, cheng2023boxteacher, li2023sim, Lan_2023_CVPR}.  
To train an instance segmentation model with box-supervision, these methods utilize a tight bounding box prior which implies that the foreground object should touch all four sides of this bounding box.
This assumption has been formulated through multiple instance learning loss~\cite{hsu2019weakly, lan2021discobox, cheng2023boxteacher, Lan_2023_CVPR}, or box-projection loss~\cite{tian2021boxinst, li2022box}. 
Additionally, to complement this formulation, several works have incorporated low-level color pairwise information~\cite{tian2021boxinst}, energy function~\cite{li2022box}, semantic information~\cite{li2023sim}, or a teacher-student framework~\cite{cheng2023boxteacher, Lan_2023_CVPR}, further narrowing the performance gap with fully supervised techniques.

% 3문단, box-supervised method들이 놓치고 있는것을 설명.
% Feedback : 두괄식으로 작성. 
% In this work, we highlight that previous research has neglected certain byproducts encountered in practical situations of annotating bounding boxes.
In this work, we utilize extreme points for the weakly supervised instance segmentation, which are byproducts encountered in practical situations of annotating bounding boxes, that has been neglected at previous research.
In a recent bounding box annotation scenario, annotators are instructed not to click on the top-left and right-most corner points of a bounding box (red dots in Fig.~\ref{fig:teaser}(a)), but rather on the extreme points of the target object: topmost, leftmost, bottommost, and rightmost points (red dots in Fig.~\ref{fig:teaser}(c)). \LHJmodified{change the describing order} 
Since being proposed by Papadopoulos et al~\cite{papadopoulos2017extreme}, this annotation scheme has been recognized as the most efficient method for creating bounding box annotations and has even been utilized in the construction of the Open Image dataset~\cite{kuznetsova2020open}. \LHJmodified{(most is to overclame)}
%최근 데이터셋 구축에 활용되어지고도있다 의 뉘앙스로 넣기 (위 문장은 그래서 어쩔건데라는느낌임)
These extreme points provide stronger information about the appearance of the target object than corner points, as they are located on the boundary of an object. Despite their potential utility, they have not received much attention in the context of box-supervised instance segmentation tasks.

% 4문단 EXITS 구조에 대한설명
Motivated by these insights, we present EXITS, an extreme point supervised instance segmentation framework. 
%갑자기 2stage 갈겨버리는거 이상함. extreme point를 활용한다는 측면에서 어떤 내용을 적어주면좋을거같음.
%exit는 extreme point를 initial labeling seed로 해서 더 나은 extreme point 활용한ㄷ. (위아래 두문장사이에, extreme point를 더 좋게 활용한다는 그런 문장이 들어갔으면 좋겠다.)
Specifically, EXITS is a two-stage framework, where the first stage aims to train a pseudo label generator for each instance annotated by extreme points, and the second stage utilizes generated pseudo masks for fully supervised learning. The overall framework is illustrated as in \Fig{stage}. 
Thanks to its flexible design, any existing instance segmentation model can be adopted for the second stage.

% 5문단 extreme point를 어떻게 활용할것인지에 대한 설명. 
Our key focus is on how to train the pseudo label generator from extreme points.
One naïve approach is using extreme points as foreground supervision and points outside the bounding box derived from extreme points as background supervision. 
However, this is inadequate for generating crisp object masks, as most regions within the bounding box remain unlabeled.
To address this issue, we retrieve points within the bounding box by propagating labels from extreme and background points based on the semantic similarity of points. 
% This could be achieved with a random walk algorithm~\cite{lovasz1993random}; however, to construct a transition probability matrix that encodes semantic similarity, we exploit the attention matrix from the multi-head self-attention mechanism in the transformer block~\cite{dosovitskiy2020image}. 
We assume that points belonging to the foreground object will be propagated from extreme points with high probability and from background points with low probability. 
Conversely, points belonging to the background are likely to be propagated from background points with high probability and from extreme points with low probability. 
Following this assumption, we retrieve points based on propagation results, and these points serve as additional supervision for training the pseudo label generator.

Our pseudo label generator generates high-quality pseudo masks even for separated objects due to severe occlusion (Fig.~\ref{fig:teaser}(d)), in contrast to a box-supervised pseudo labeler~\cite{Lan_2023_CVPR}, which struggles in the same conditions (Fig.~\ref{fig:teaser}(b)). 
%이거 좀더 깔끔하게 이야기하기.
%이 아래문장은, 우리는 extrmee point를 활용한 덕분에, 사전연구가 주로 의존하는 BBTP 가정에 의존하지 않을수있기때문이다. 이런 느낌으로 들어가는게 나을거같음. 그뒤에 onthe otherhand말고 BBTP 가정이 왜 안되는지 이야기해줄수 있을거같음. 
The effectiveness of our approach stems from the point retrieval algorithm, which provides a delicate supervisory signal about the target object. 
On the other hand, box-supervised methods rely on a weaker assumption, the tightness of the bounding box prior, which often proves insufficient in complex scenes. 
To quantitatively compare the quality of pseudo labels for separated objects, we measured the pseudo label quality on the Separated COCO dataset~\cite{zhan2022tri}. 
%Seprated coco dataset 좀더 설명하기 (which is subset of coco val set 등으로)
Our approach outperforms previous work~\cite{Lan_2023_CVPR} by an impressive margin of 7 mIoU. 
% 좀더 덤덤하게 적기? 
Furthermore, extensive experiments are conducted on three public benchmarks to demonstrate the superiority of our approach, outperforming all the previous box-supervised instance segmentation methods. 

In short, the main contribution of this paper is four-fold:
\begin{itemize}
    \item We propose to utilize extreme points for weakly supervised instance segmentation. Extreme points can be obtained during bounding box annotations without extra costs.
    \item We introduce a point retrieval algorithm, which effectively leverages extreme points to estimate labels of points in the bounding box. Specifically, this algorithm estimates the labels of points based on the probability of propagation to extreme points and background points. 
    \item Our method generates high-quality pseudo masks, particularly for separated objects, unlike those trained with box supervision which struggle to generate accurately in these cases.
    \item Our proposed framework achieved state-of-the-art performance on three public benchmarks with a significant margin under the same labeling cost.
\end{itemize}







%instance segmentation model 설명
%box-supervised method에 대해 설명, Multiple instance learning에 대해 설명.
%extreme point를 도입하고자 한다. (extreme point는 annotation cost -> box보다 쉬움, 좌상단 우하단 클릭하는 것보다 빠름.)


% 1. instance segmentation model에 대한 설명 / weakly-supervised 방식들 또한 생겨내게 됨을 설명
% 2. 

\label{sec:intro}





% To insert a figure: \input{figs/template}
% Or table: \input{tables/template}https://www.overleaf.com/project/6523d5cc7d6718c1ac3e2d88

==> sections/01_intro_backup_1117.tex <==
\section{Introduction}

%문단 구조 나누기. 핵심 내용 적기.
%1. instance segmentation 모델에 대한 설명. + instance segmentation task의 중요성 + weak sup 방식들이 나오게 된 이유.
%This technique is particularly invaluable in domains such as autonomous driving, robotic manipulation, and medical image analysis, where identifying specific entities like people, vehicles, and tumors is crucial.
Instance segmentation, a foundational task in computer vision, has made significant strides through supervised learning of deep neural networks~\cite{mask_rcnn, wang2020solo, wang2020solov2, tian2020conditional, cheng2022masked}. 
However, its broader application is hindered since the required pixel-level masks are prohibitively expensive to obtain. thereby driving the pursuit of the weakly supervised approach. 
% 사실 이렇게 끝나지 않으면 어색함. 만약 다른 방식들을 나열하고 box-supervised learning method 설명으로 넘어가는게 살짝 어색하긴함. HMMMM 일단 보류. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/Teaser_8.png}
    \end{subfigure}
    \caption{\textbf{Types of weak supervision for instance segmentation and their corresponding generated pseudo labels.} Top: A box-supervised method~\cite{Lan_2023_CVPR} struggles to generate an accurate pseudo label for the separated object. Bottom: Our approach leverages extreme points as weak supervision, attainable during the box annotation process at no extra cost, and generates a precise pseudo label for the separated object. Best viewed in color.}
    \label{fig:teaser}
    \vspace{-3mm}
\end{figure}

%2문단, box-supervised model에 대한 설명. 

Building on this momentum, research about box-supervised instance segmentation has gained considerable traction~\cite{khoreva2017simple, lee2021bbam, hsu2019weakly, tian2021boxinst, lan2021discobox, li2022box, cheng2023boxteacher, li2023sim, Lan_2023_CVPR}.  
To train an instance segmentation model with box-supervision, these methods utilize a tight bounding box prior~\cite{hsu2019weakly} which implies that a vertical (or horizontal) line crossing the bounding box must contain at least one pixel belonging to the object.
This assumption has been formulated through multiple instance learning loss~\cite{hsu2019weakly, lan2021discobox, cheng2023boxteacher, Lan_2023_CVPR}, or box-projection loss~\cite{tian2021boxinst, li2022box}. 
Additionally, to complement this formulation, several works have incorporated low-level color pairwise information~\cite{tian2021boxinst}, energy function~\cite{li2022box}, semantic information~\cite{li2023sim}, or a teacher-student framework~\cite{cheng2023boxteacher, Lan_2023_CVPR}, further narrowing the performance gap with fully supervised techniques.

% 3문단, box-supervised method들이 놓치고 있는것을 설명.
In this work, we tackle weakly supervised instance segmentation using extreme points, which are neglected byproducts of the bounding box annotation process. 
Under the recent paradigm of bounding box annotation, annotators are instructed to click extreme points of the target object: topmost, leftmost, bottommost, and rightmost points (red dots in Fig.~\ref{fig:teaser}(c)), rather than to click two corner points of bounding box (red dots in Fig.~\ref{fig:teaser}(a)). 
Since being proposed by Papadopoulos et al~\cite{papadopoulos2017extreme}, this annotation process has been recognized as an efficient method for labeling bounding box and has been adopted in recent dataset construction, such as Open Image~\cite{kuznetsova2020open}. 
Thus, extreme points can be freely obtained during the practical bounding box annotation process, and furthermore, these points provide a strong clue about the appearance of the target object as they are located on the boundary of an object.
Despite their potential utility, they have not received much attention in the context of box-supervised instance segmentation tasks.

% 4문단 EXITS 구조에 대한설명
Motivated by these insights, we present EXITS, an extreme point supervised instance segmentation framework. 
EXITS utilizes extreme points as initial seed labels and employs label propagation to provide additional supervision for segmentation.
Specifically, EXITS is a two-stage framework, where the first stage aims to train a pseudo label generator for each instance annotated by extreme points, and the second stage utilizes generated pseudo masks for fully supervised learning. The overall framework is illustrated as in \Fig{stage}. 
Thanks to its flexible design, any existing instance segmentation model can be adopted for the second stage.

% 5문단 extreme point를 어떻게 활용할것인지에 대한 설명. 
Our key focus is on how to train the pseudo label generator from extreme points.
One naïve approach is using extreme points as foreground supervision and points outside the bounding box derived from extreme points as background supervision. 
However, this is inadequate for generating crisp object masks, as most regions within the bounding box remain unlabeled.
To address this issue, we retrieve points within the bounding box by propagating labels from extreme and background points based on the semantic similarity of points. 
We assume that points belonging to the foreground object will be propagated from extreme points with high probability and from background points with low probability. 
Conversely, points belonging to the background are likely to be propagated from background points with high probability and from extreme points with low probability. 
Following this assumption, we retrieve points based on propagation results, and these points serve as additional supervision for training the pseudo label generator.

% Our pseudo label generator generates high-quality pseudo masks even for separated objects due to severe occlusion (Fig.~\ref{fig:teaser}(d)), in contrast to a box-supervised pseudo labeler~\cite{Lan_2023_CVPR} often fails (Fig.~\ref{fig:teaser}(b)).
Our pseudo label generator generates high-quality pseudo masks even for separated objects due to severe occlusion (Fig.~\ref{fig:teaser}(d)), where the conventional methods often fail (\Fig{teaser}(b)) due to their underlying tight bounding box prior.
% This is because box-supervised methods often rely on the tight bounding box prior which is insufficient in the case of separated objects.
They assume that a vertical (or horizontal) line crossing the bounding box must contain at least a single pixel belonging to the object, which is often violated in the case of separated objects.
% which is insufficient in the case of separated objects.
As shown in pictures in~\Fig{teaser}, a vertical line passing through the tree trunk does not contain any of the foreground (car) pixels.
% Thanks to employing extreme points and point retrieval algorithms using these points, EXITS does not heavily rely on the weak assumption, the tight bounding box prior.
% Thanks to employing extreme points and point retrieval algorithms using these points, EXITS does not heavily rely on the weak assumption, the tight bounding box prior.
Thanks to the proposed point retrieval algorithms utilizing the extreme points, EXITS allows to train segmentation model without heavily relying on the tight bounding box prior.
% \LHJmodified{Or, It estimate label of pixel belonging to the tree trunk (occluder) as background by propagation through semantic similarity.}
% Thanks to the point retrieval algorithm, which provides a delicate supervisory signal about the target object. 
% On the other hand, box-supervised methods rely on a weaker assumption, the tightness of the bounding box prior, which often proves insufficient in complex scenes. 

To quantitatively compare the quality of pseudo labels for separated objects, we measured the pseudo label quality on the Separated COCO dataset~\cite{zhan2022tri}, which is a subset of the COCO~\cite{Mscoco} comprising only separated objects.
In Separated COCO, our method demonstrates significant improvement, surpassing previous work~\cite{Lan_2023_CVPR} with a 7.2 mIoU.
% Furthermore, extensive experiments for instance segmentation task are conducted on three public benchmarks to demonstrate the superiority of our approach, outperforming all the previous box-supervised instance segmentation methods.
Furthermore, to demonstrate the superiority of EXITS, extensive experiments are conducted on three public benchmarks: PASCAL VOC~\cite{Pascalvoc}, COCO, LVIS~\cite{gupta2019lvis}, where EXITS outperforms all the previous box-supervised instance segmentation methods.

In short, the main contribution of this paper is four-fold:
\begin{itemize}
    \item We propose to utilize extreme points for weakly supervised instance segmentation. Extreme points can be obtained during bounding box annotations without extra costs.
    \item We introduce a point retrieval algorithm, which effectively leverages extreme points to estimate labels of points in the bounding box.
    Specifically, this algorithm estimates the labels of points based on the probability of propagation to extreme points and background points. 
    \item Our method generates high-quality pseudo masks, particularly for separated objects, unlike those trained with box supervision which struggle to generate accurately in these cases.
    \item Our proposed framework achieved state-of-the-art performance on three public benchmarks with a significant margin.
\end{itemize}







%instance segmentation model 설명
%box-supervised method에 대해 설명, Multiple instance learning에 대해 설명.
%extreme point를 도입하고자 한다. (extreme point는 annotation cost -> box보다 쉬움, 좌상단 우하단 클릭하는 것보다 빠름.)


% 1. instance segmentation model에 대한 설명 / weakly-supervised 방식들 또한 생겨내게 됨을 설명
% 2. 

\label{sec:intro}





% To insert a figure: \input{figs/template}
% Or table: \input{tables/template}https://www.overleaf.com/project/6523d5cc7d6718c1ac3e2d88

==> sections/03_method_backup_231110.tex <==
\section{Proposed Method}

\begin{figure*}[t]
    \centering
        \includegraphics[width=\textwidth]{figures/overall_pipeline_v2.pdf}
        \caption{\hsh{Overview of EXITS framework.
                The model is trained on images \LHJ{cropped to include background pixels around the individual object, aiming to predict binary masks}.
                Training leverages three loss functions: $\mathcal{L}_\text{crf}$ aligns images before and after CRF~\cite{crf} processing, $\mathcal{L}_\text{mil}$ ensures a foreground predicted pixel exists in every row and column of the bounding box, and $\mathcal{L}_\text{point}$ uses extreme points-derived pseudo labels for precise pixel-wise supervision.
                To generate these pseudo points, EXITS obtains initial foreground and background points from extreme points, then employs self-attention of warm-up trained ViT as a transition matrix for label propagation.
                After propagation, \LHJ{point-wise labels are produced based on the difference of propagation score to the foreground and background,} from which some are dropped out to form the final set of pseudo-point labels.}}
                % Pseudo-point labels are initially generated from extreme points, with the self-attention of warm-up trained VIT facilitating label propagation.
                % The resulting pseudo-point labels are dynamically dropped out to establish the final set of pseudo-point labels.}}
    \label{fig:pipeline}
\end{figure*} 
% Notation으로 setting 적어주기.
% 우리는 Stage 1, Stage 2로 나누어서 진행한다.
% Stage 1 에서는 extreme point로부터  cropped input image 를 받아 해당 object에 해당하는 pseudo mask를 생성하는 netowrk를 학습한다.
% Stage 2는 stage 1에서부터 얻은 pseudo mask를 gt-mask로 취급하여 fully-supervised instance segmentation model들을 학습한다. 
% 우리는 Stage 1에 더 집중하여 이를 설명하고자 한다. 
% 먼저, extreme point에 대한 설명은 3.1에, extreme point로부터 pseudo label를 생성하는 방식에 대해서는 3.2, 3.3에 설명하려고 한다. 
\iffalse
Our approach to weakly supervised instance segmentation is divided into two stages: (1) Generating pixel-wise segmentation labels of each object annotated by extreme points, and (2) Learning DNN for instance segmentation with the generated pseudo labels by the first stage. 
In the first stage, the segmentation model receives images that have been cropped around objects annotated by extreme points. It is then trained to predict the corresponding object mask supervised by reachable points from extreme points and background points as ~\Fig{pipeline}. 
In the second stage, we can apply any fully supervised instance segmentation pipeline~\cite{wang2020solov2, cheng2022masked} using pseudo label generated by the first stage. Therefore, we will focus on describing the first stage. 
\fi
\hsh{
Our approach to weakly supervised instance segmentation is divided into two stages: (1) Generating pixel-wise segmentation labels of each object annotated by extreme points, and (2) Learning DNN for instance segmentation with the generated pseudo labels by the first stage. 
In the first stage, the segmentation model receives images that have been cropped around objects annotated by extreme points. It is then trained to predict the corresponding object mask supervised by reachable points from extreme points and background points as ~\Fig{pipeline}. 
In the second stage, we can apply any fully supervised instance segmentation pipeline~\cite{wang2020solov2, cheng2022masked} using pseudo label generated by the first stage. Therefore, we will focus on describing the first stage. 
}

 The remainder of this section describes the preliminary of extreme points (Sec.~\ref{subsec:subsection2}), and how to train the segmentation model to generate object masks from corresponding extreme points (Sec.~\ref{subsec:subsection4}, Sec.~\ref{subsec:subsection5}). 


%In the setting of weakly supervised instance segmentation, we are given a set of extreme points annotated training data \mathcal{D} = \{(X_n, Y_n, B_n)\}_{n=1}^{N}. 
%Notation : 
%original image : $\textbf{I}$, cropped image : $\textbf{I}^c$, extreme points in cropped image $ \textbf{e} = \{ (x^{(t)}, y^{(t)})$, $(x^{(l)}, y^{(l)})$, $(x^{(b)}, y^{(b)})$, $(x^{(r)}, y^{(r)}) \}$, 

% 우리의 전반적인 Pipeline은 다음과 같다. (그림 ~와 같다)
% 우리는 extreme point로부터 얻을수 있는 bounding box 로부터 cropping 한 region을 input으로 받고, 그에 해당하는 object의 mask를 예측하는 network를 학습하고자 한다.
% 이는 object를 한번에 하나씩 처리할수 있으며, given bounding box 안의 object를 예측하는것으로 문제를 streamline 할 수 있다.
% cropped image input으로 pseudo label을 생성하는 network를 학습한뒤, pseudo labeling 을 한 뒤에 fully supervised instance segmentation model을 학습하는 방식이다. 
% 

%좀더 매트하게 적기. 
\subsection{Preliminary: Extreme Points}
\label{subsec:subsection2}


Extreme points are defined as the outermost points on an object along the cardinal directions: the topmost point $(x^{(t)}, y^{(t)})$, the leftmost point $(x^{(l)}, y^{(l)})$, the bottommost point $(x^{(b)}, y^{(b)})$, rightmost point $(x^{(r)}, y^{(r)})$. Papadopoulos \etal \cite{papadopoulos2017extreme} has shown that clicking these points is a more efficient approach to bounding box annotation compared to the conventional method of clicking the top-left $(x^{(l)}, y^{(t)})$ and bottom-right $(x^{(r)}, y^{(b)})$ points of a rectangular area that encompasses the target object. The latter often leads to inaccuracies because corner points do not correspond to the actual features of the object, requiring the annotator to make additional adjustments and taking an average of 34.5 seconds per object. In contrast, extreme point clicking reduces annotation time to 7.2 seconds per object.
Thus, extreme point annotation effectively comes at no extra cost when performing bounding box labeling, as these points can be effortlessly marked in the process. Additionally, since extreme points lie on the object's boundary, they inherently provide more information about the appearance of the target object compared to the two corner points of a bounding box.

% \subsection{Naïve Way to Learning with Extreme Points}
% % 우리는 extreme point 의 geometric 한 특성으로부터 annotation으로 부터 다음과 같은 내용을 유추할수 있다.
% % 1) Extreme point는 각 cardinal direction의 boundary point이다. 이는 다시말해 해당 point들을 각 bounding box에 orthogonal 방향에는 target object에 해당하는 foreground point가 존재한다. 
% % 2) Extreme point로부터 그릴 수 있는 bounding box의 outside에 해당하는 점들은 target object와 구별되는 확실한 background point이다. 
% % 위의 두 내용을 바탕으로, Exrtreme Point를 가장 straightforward하게 weak supervision으로써 활용하는 방식은 다음과 같다. 각 extreme point 를 이로부터 얻을수 있는 bounding bos에 orthogonal 한 방향으로 이동시킨점을 4개의 foregrond point로 간주하고, bounding box 바깥의 점들을 background point로 간주하여 direct supervision을 적용한다. 
% From the geometric characteristics of extreme points, we can deduce the relationship between the target object and the extreme points as follows:
% \textbf{First}, each extreme point represents a boundary point in its cardinal direction, which implies that orthogonal to each point within the corresponding bounding box, there exists a foreground point about the target object. 
% we will call these points as initial foreground points $ \mathcal{P}_{\textrm{FG}} \in \{ (x^{(t)}, y^{(t)}-\delta)$, $(x^{(l)}+\delta, y^{(l)})$, $(x^{(b)}, y^{(b)}+\delta)$, $(x^{(r)}-\delta, y^{(r)}) \}$.
% \textbf{Second}, points outside the bounding box drawn from extreme points are definitive background points, distinct from the target object. we call these points as certain background points $\mathcal{P}_{\textrm{BG}}.$
% Based on these premises, the naïve way of utilizing extreme points as weak supervision is using $ \mathcal{P}_{\textrm{FG}} , \mathcal{P}_{\textrm{BG}}$ as point-wise supervision for binary segmentation.

% % 그러나, 해당 방식은 여전히 bounding box 내부의 대부분의 region을 학습에 사용하지 않기 때문에 fine-grained 한 object mask를 생성해 낼 수없다. 
% %= 그에 대한 결과로써 bounding box로 줄 수 있는 supervision인 Mulitple Instance Learning loss를 사용한 것보다 성능이 오히려 떨어지는 경향성을 초래한다. 
% % 그러나, 해당 lack of information about how object appears (or located) in bounding box,
% % fine-grained 한 object mask를 생성해 낼 수없다. 그 결과로써, bounding box 방식들이 사용하는 MIL loss를 적용했을때 보다 낮은 성능을 보이기도 한다. 
% %우리는 extreme point 으로 부터 더 풍부한 supervision을 학습에 제공하기 위해, 다음과 같은 가정을 통해 추가적인 supervision을 제공하고자 한다.
% % 이미지위의 point들을 하나의 그래프로 가정하고, 이를 propagation 시켰을때 
% % bounding box내부의 point 들 중, target object 위에 해당하는 point 들은 initial Foreground points 로 propagation 될 확률은 높을것이고, certain background points로 propagation 확률은 낮을것 이다. 
% % 또한 그와 마찬가지로 box 내부의 point들 중, target object 밖에 해당하는 point 들은 certain background points 로 transition 될 확률은 높을것이고, initial foreground  points로 transition 확률은 낮을것이다.
% % 우리는 이 가정에 기반하여, bounding box 내부의 reachable point들을 골라 이를 추가적인 supervision으로 활용한다

% However, the majority of the region within the bounding box remains ambiguous, thereby offering no clear supervisory signal. Consequently,  solely relying on $\mathcal{P}_{\textrm{FG}}$,  $\mathcal{P}_{\textrm{BG}}$ for training is inadequate for predicting a fine-grained object mask.
% %Consequently, this approach might underperforms compared to bounding box-based methods that utilize Multiple Instance Learning (MIL) loss. \LHJ{(add ablation study to support this sentence)} 
% To provide richer supervision from extreme points for training, we aim to offer additional supervision for the points within the bounding box based on the following assumption:
% When propagating points in an image, those within the bounding box that lie on the target object are likely to propagate to $\mathcal{P}_{\textrm{FG}}$ with a high probability, while their probability of propagating to $\mathcal{P}_{\textrm{BG}}$ will be low. 
% Similarly, points within the bounding box that lie in the background are expected to propagate to $\mathcal{P}_{\textrm{BG}}$ with a high probability, and to $\mathcal{P}_{\textrm{FG}}$ with a low probability.
% Building on this assumption, we select reachable points within the bounding box to leverage them as additional supervision.

\subsection{Learning to Generate Mask from Extreme Points}
\label{subsec:subsection4}

From the geometric characteristics of extreme points, we can deduce the relationship between the target object and the extreme points as follows:
\textbf{First}, each extreme point represents a boundary point in its cardinal direction, which implies that orthogonal to each point within the corresponding bounding box, there exists a foreground point about the target object. 
we will call these set of points as initial foreground points set $ \mathcal{P}_{\textrm{FG}} \in \{ (x^{(t)}, y^{(t)}-\delta)$, $(x^{(l)}+\delta, y^{(l)})$, $(x^{(b)}, y^{(b)}+\delta)$, $(x^{(r)}-\delta, y^{(r)}) \}$.
\textbf{Second}, points outside the bounding box drawn from extreme points are definitive background points, distinct from the target object. we call these set of points as certain background points set $\mathcal{P}_{\textrm{BG}}.$
Based on these premises, the naïve way of utilizing extreme points as weak supervision is using $ \mathcal{P}_{\textrm{FG}} , \mathcal{P}_{\textrm{BG}}$ as point-wise supervision for binary segmentation.

However, the majority of the region within the bounding box remains ambiguous, thereby offering no clear supervisory signal. Consequently,  solely relying on $\mathcal{P}_{\textrm{FG}}$,  $\mathcal{P}_{\textrm{BG}}$ for training is inadequate for predicting a fine-grained object mask.
%Consequently, this approach might underperforms compared to bounding box-based methods that utilize Multiple Instance Learning (MIL) loss. \LHJ{(add ablation study to support this sentence)} 
To provide richer supervision from extreme points for training, we aim to offer additional supervision for the points within the bounding box based on the following assumption:
When propagating points in an image, those within the bounding box that lie on the target object are likely to propagate to $\mathcal{P}_{\textrm{FG}}$ with a high probability, while their probability of propagating to $\mathcal{P}_{\textrm{BG}}$ will be low. 
Similarly, points within the bounding box that lie in the background are expected to propagate to $\mathcal{P}_{\textrm{BG}}$ with a high probability, and to $\mathcal{P}_{\textrm{FG}}$ with a low probability.
Building on this assumption, we select reachable points within the bounding box to leverage them as additional supervision.

% 우리는 image encoder, decoder architecture를 사용한다.
% image encoder 구조는 vision transformer architecture를 사용하는데, 이에 감사하게도, vision transformer의 multi head sefl attention으로 부터 transition probability matrix를 만들었다. 
%MHSA 로부터 Transition probability matrix를 만든 이유는 다음과 같다. 
%1) MHSA is pair-wise affinity contains high-level semantic information 이다. 이는 point를 propagation 시키는데 있어, apprearnce가 비슷하지만 다른 semantic으로 propagation 되는것을 방지해줄수 있다. (low-level image cue like color-pairwise affinity로 이를 만들었다면, Figure 1처럼 pseudo label 만들지 못할것임. 
%2) multi head self attention 은 global feature ependency 를 고려할수 있다. 즉, 이를 통해 만들어진 TPM은 point를 local한 부분으로만 propagation 하도록 제한하지 않는다.
%이는 point propagation이 object가 separated 된 케이스에 대해서도 잘 일어날수 있게 해준다. 

\subsubsection{Constructing Transition Probability Matrix}
To propagate points, we construct a Transition Probability Matrix (TPM) from the Multi-Head Self-Attention (MHSA) in the transformer block. 
Specifically, cropped image $I^c \in \mathbb{R}^{H \times W}$ is firstly split into $N$ patches, where each patch is flattened and linearly projected.
These patches serve as the input for a vision transformer $E^{\text{p}}$, where the MHSA in the $i$-th transformer block is denoted as $\mathbf{S}_i \in \mathbb{R}^{N \times N}$. 
We use the 10th transformer block's MHSA $(i=10)$ to balance detail and high-level semantics, as earlier blocks easily miss high-level semantics and later blocks tend to over-smooth patch representation~\cite{Ru_2023_CVPR}.


However, since the queries and keys used to create $\mathbf{S}_i$ are projected from different layers, $\mathbf{S}_i$ is inherently asymmetric. We wish the TPM should be symmetric, meaning that the transition probability from point $p_i$ to point $p_j$ should be equal the probability from point $p_j$ to point $p_i$.
 Given the affinity matrix $\mathbf{S}_i$ from MHSA, we can calculate a symmetric transition probability matrix $\mathbf{T}$ using the following formula,

\begin{equation}\label{eqn:eq2}
    \mathbf{T} = \frac{\mathbf{A} + \mathbf{A}^\top}{2},   \text{  where  } \mathbf{A} = \text{Sinkhorn}(\mathbf{S}_i)
\end{equation}

\noindent where $\text{Sinkhorn}(\cdot)$ refers to the Sinkhorn-Knopp algorithm ~\cite{knight2008sinkhorn}, which is employed to transform a matrix into a doubly-stochastic form.

% Following this, the transition probability matrix \matbhf{T} with $\alpha$ hops can be defined as  
% \begin{equation}\label{eqn:eq2}
%     \mathbf{T} = \mathbf{A}^\alpha
% \end{equation}

\noindent \textbf{Warm-up} Before generating TPM, we warm up the $E^{\text{p}}$ to enhance its ability to differentiate between the background and the target object. Specifically, for the predicted mask probability map $\mathcal{M'}$ obtained through ViT Encoder $E^{\text{p}}$ and auxiliary decoder  $D^{\text{auc}}$, we employ the Multiple Instance Learning (MIL) loss as follow :

\begin{equation}
\label{eq:mil_loss}
\begin{aligned}
\mathcal{L}_{\text{mil}} = \mathcal{L}_{\text{dice}}(&\max_{x}(\mathcal{M}'), \max_{x}(\mathcal{M}_{\text{box}})) \\
&+ \mathcal{L}_{\text{dice}}(\max_y(\mathcal{M}'), \max_y(\mathcal{M}_{\text{box}}))
\end{aligned}
\end{equation}

\noindent where $\max_{x}, \max_y$ indicate max operation along x, y axis, and $\mathcal{L}_{\text{dice}}$ indicates dice loss~\cite{sudre2017generalised}. $\mathcal{M}_{\text{box}} \in \{0,1\}^{H\times W}$ indicates box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise. Note that $D^{\text{auc}}$ is only used for warm-up.

\noindent \textbf{Why TPM from MHSA?}  The extraction of a TPM from the MHSA is beneficial for several reasons. MHSA captures pairwise affinity that contains high-level semantic information. This helps to prevent points from being propagated to other points with a similar appearance but different semantics.
Additionally, MHSA reflects a matrix embodying global feature dependencies, enabling the TPM constructed through it to facilitate point propagation beyond local areas. This allows for the propagation of points across separated segments of an object.

\subsubsection{Point selection algorithm}

% Probability FG = average 
 % probability BG = average
 % probdifference 에 기반해서 point i 의 pseudo label 부여

% Let us denote the set of points within the bounding box that can be drawn from extreme point as $\mathcal{P}_{\text{Box}}$. 
% Our objective is to assign pseudo label of points $i \in \mathcal{P}_{\text{Box}}$ based on their tendency of propagation 
% to the foreground points set $\mathcal{P}_{\text{FG}}$ and background point set $\mathcal{P}_{\text{BG}}$.

% We define the tendency of point $i$ to propagate to$\mathcal{P}_{\text{FG}}$ as the average probability among points $j \in \mathcal{P}_{\text{FG}}$
    
Let's denote the set of points within the bounding box that can be drawn from the extreme point as $\mathcal{P}_{\text{Box}}$. Our goal is to assign a pseudo label to points $p_i \in \mathcal{P}_{\text{Box}}$ based on their tendency to propagate towards the foreground points set $\mathcal{P}_{\text{FG}}$ and the background point set $\mathcal{P}_{\text{BG}}$.

We define the probability score for point $p_i$ to propagate towards $\mathcal{P}_{\text{FG}}$ as the average probability of its propagation to each of the four foreground points :

\begin{equation}
\pi_i^{\text{FG}}
 = \frac{1}{|\mathcal{P}_{\text{FG}}|} \sum_{p_j \in \mathcal{P}_{\text{FG}}} \mathbf{T}^\alpha(i, j)
\end{equation}

\noindent where $\mathbf{T}^\alpha(i, j)$ represents the transition probability that point 
$p_i$ will propagate to point $p_j$ through $\alpha$ hops.

Similarly, we define the probability score for point \(p_i \) to propagate towards \( \mathcal{P}_{\text{BG}} \) in an analogous manner. The score is computed as the average probability of point \( p_i \)'s propagation to each of the background points:

\begin{equation}
\pi_i^{\text{BG}}
 = \frac{1}{|\mathcal{P}_{\text{BG}}|} \sum_{p_k \in \mathcal{P}_{\text{BG}}} \mathbf{T}^\alpha(i, k)
\end{equation}

Based on the probability scores to $\mathcal{P}_{\text{FG}}$ and $\mathcal{P}_{\text{BG}}$, the assigned pseudo label for point $p_i \in \mathcal{P}_{\text{Box}}$ is estimated by 

\begin{equation}
\hat{y}_i =
\begin{cases}
1, & \text{if } \pi_i^{\text{FG}} - \pi_i^{\text{BG}} \geq \tau_{fg} \\
0, & \text{if } \pi_i^{\text{FG}} - \pi_i^{\text{BG}} \leq \tau_{bg} \\
\text{unlabeled}, & \text{otherwise}
\end{cases}
\end{equation}

\noindent where $\tau_{fg}, \tau_{bg}$ are the hyperparameters used to filter out ambiguous points.

\noindent \textbf{Point drop out}
To enhance diversity and prevent overfitting, we adopt a point drop out strategy as an augmentation technique. Within each epoch, for the set of selected points $p_i \in \mathcal{P}_{\text{Box}}$, we randomly drop \( n\% \) of the points and do not use them as supervision. This selective drop-out is applied separately to the foreground-labeled point and background-labeled point sets, ensuring that each maintains a dynamic and balanced representation throughout the learning process.




\noindent \subsection{Objective Function}
\label{subsec:subsection5}


\LHJ{HJ : explain example sample of MIL adopted sample, should I explain about masking strategy for unlabeled point region?} 

\noindent \textbf{Point Loss}
We construct binary mask $\mathcal{\hat{Y}}$ using set of points $\mathcal{P}_{\text{FG}} \cup \mathcal{P}_{\text{BG}} \cup \mathcal{P}_{\text{labeled}}$, where $\mathcal{P}_{\text{labeled}} = \{ p_i \mid p_i \in \mathcal{P}_{\text{Box}}, \hat{y}_i \neq \text{unlabeled} \} $.
We use dice loss between $\mathcal{\hat{Y}}$ between predicted mask probability $\mathcal{M}$ for the point loss. However, there are cases where points cannot be selected using the point selection algorithm. ($ | \mathcal{P}_{\text{labeled}} | = 0 $) For these samples, we applied an additional MIL loss used in Eq ~\ref{eq:mil_loss}.
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{point}} =  \mathcal{L}_{\text{dice}}(\mathcal{M},\mathcal{\hat{Y}}) + \mathds{1}_{\{|\mathcal{P}_{\text{labeled}}| = 0\}} \lambda_{mil} \mathcal{L}_{\text{mil}}
\end{aligned}
\end{equation}

\noindent where $\mathds{1}$ is indicator function. 
Note that samples subjected MIL loss account for only about $7\%$ of the entire sample, so our framework does not heavily depend on MIL loss.

\noindent \textbf{CRF Loss with self training} \LHJ{TODO}


\noindent Formally, the overall loss function of EXITS can be formulated as :
\begin{equation}
\begin{aligned}
\mathcal{L}_{overall} =  \lambda_{point} \mathcal{L}_{\text{point}} +  \lambda_{crf} \mathcal{L}_{\text{crf}} 
\end{aligned}
\end{equation}








% method 흐름 
% StraightForward but effective
% 사전 work (MAL) 에 쓰이는 테크닉들은 가볍게 언급정도로만 하기. ex) CRF loss, EMA teacher
% 스페시픽하게 적어야 하는 내용들은 내가 발전시킨 부분들. 꼭 들어가야 하는 내용들? 
% 1) How to construct Transition Probability Matrix?
%    (a) input image fed into ViT encoder , Multihead self attention.
%    (b) What is the index of Transition Probability Matrix is needed.  
% 2) How to select certain Foreground and Background points in the bounding box 
%    (a) sampling strategy? 
%    (b)
% 3) How to train with selected Point? How to justify dice loss between point label and dice loss? 
% 4) additional loss - self-refinement scheme (CRF loss),MIL loss for no point selected in the image. 

%in section 3.1 
%필요한 수식들 정리해놓기. 

==> sections/03_method_backup_231114.tex <==
\section{Proposed Method}

%Feedback : Stage 1 인거 명시적으로 설명해주기. 
\begin{figure*}[t]
    \centering
        \includegraphics[width=\textwidth]{figures/overall_pipeline_v2.3.pdf}
        \caption{\hsh{\LHJ{Overview of stage 1 in EXITS framework}.
                The pseudo label generator is trained on images \LHJ{cropped to include background pixels around the extreme points, aiming to predict binary masks}.
                Training leverages two loss functions: $\mathcal{L}_\text{crf}$ aligns images before and after CRF~\cite{crf} processing,
                % $\mathcal{L}_\text{mil}$ ensures a foreground predicted pixel exists in every row and column of the bounding box,
                and $\mathcal{L}_\text{point}$ uses extreme points-derived pseudo labels for precise pixel-wise supervision.
                To generate these pseudo points, EXITS obtains initial foreground and background points from extreme points, then employs self-attention of warm-up trained ViT as a transition matrix for label propagation.
                After propagation, \LHJ{point-wise labels are produced based on the difference of propagation score to the foreground and background,} from which some are dropped out to form the final set of pseudo-point labels.}}
                % Pseudo-point labels are initially generated from extreme points, with the self-attention of warm-up trained VIT facilitating label propagation.
                % The resulting pseudo-point labels are dynamically dropped out to establish the final set of pseudo-point labels.}}
    \label{fig:pipeline}
\end{figure*} 
% Feedback : 왜 pseudo labeler의 output으로는 final model prediction으로 사용할 수 없는지 설명하기. 
% Feedback : stage 2 instance segmentation model이랑 stage 1 instance segmentation model을 "명시적으로"분리해서 설명하기
\iffalse
Our approach to weakly supervised instance segmentation is divided into two stages: (1) Generating pixel-wise segmentation labels of each object annotated by extreme points, and (2) Learning DNN for instance segmentation with the generated pseudo labels by the first stage. 
In the first stage, the segmentation model receives images that have been cropped around objects annotated by extreme points \suhac{}. It is then trained to predict the corresponding object mask supervised by reachable points from extreme points and background points as~\Fig{pipeline}. 
In the second stage, we can apply any fully supervised instance segmentation pipeline~\cite{wang2020solov2, cheng2022masked} using pseudo label generated by the first stage. Therefore, we will focus on describing the first stage. 

The remainder of this section describes the preliminary of extreme points (Sec.~\ref{sec:subsection2}), and how to train the segmentation model to generate object masks from corresponding extreme points (Sec.~\ref{sec:subsection4}, Sec.~\ref{sec:subsection5}). 
\fi


\suha{Our method for EXtreme point based InsTance Segmentation, dubbed EXITS, consists of two stages: (1) learning a model that generates pseudo segmentation labels of training images using their extreme point labels, and (2) training an instance segmentation model using the pseudo labels.
 
In the first stage, an object image cropped around each object using extreme points is used as an input to the pseudo label generator so that the model learns to predict a binary mask of the object within the cropped image.
 On the other hand, the instance segmentation model in the second stage, which is our target model, learns to detect and segment multiple objects. 
Note that the pseudo label generator deals with an easier task, \ie, instance segmentation on a single object image, which enables to improve the quality of pseudo labels it generates.
The entire pipeline of EXITS is illustrated in~\Fig{stage}.

Since the second stage is the conventional supervised learning that can be applied to any instance segmentation model, this section elaborates mostly on the first stage, in particular, how EXITS provides the pseudo label generator with effective supervision for segmentation. 
The overall pipeline of the first stage is illustrated in Fig.~\ref{fig:pipeline}.
The key idea of EXITS is to retrieve pixels likely to belong to the object given the extreme points, and exploit them as (sparse) supervision for learning segmentation.
This idea is realized by propagating the extreme points to other pixels within the input object image, while considering the extreme points as a subset of true pixels of the object.

The remainder of this section first discusses extreme points and advantages of using them (\Sec{subsection1}), and then presents details of the first stage (\Sec{subsection2}) and the second stage (\Sec{subsection3}) of EXITS.
% and then presents details of point supervision generation and loss functions for learning the pseudo label generator (\Sec{subsection2}).}
% \LHJ{Lastly, we describe how the pseudo labels from first stage are integrated into existing fully supervised instance segmentation models in the second stage. (\Sec{subsection3})
}
% \hsh{
% The EXtreme point-based InsTance Segmentation (EXITS) framework operates through two stages: (1) It learns to create pixel-wise segmentation pseudo labels for training images, guided by their extreme point labels.
% (2) It employs these pseudo labels to train a fully supervised instance segmentation model.
% Since any conventional instance segmentation model can be utilized in the second stage, we focus on describing the first stage -- generating a precise pseudo-segmentation label given extreme points.

% In the first stage, the input image is cropped around each object using extreme points, and the model is trained to predict a binary mask of the input object of interest.
% Since pixel-wise segmentation labels are inaccessible, EXITS proposes to propagate foreground labels from the extreme points, and background labels from the pixels located outside of the object of interest.
% \Fig{pipeline} describes the overall pipeline of the first stage.
% The remainder of this section describes the preliminary of extreme points (\Sec{subsection2}), the pipeline of generating pseudo mask labels (\Sec{subsection4}), and our objective functions (\Sec{subsection5}).}


%In the setting of weakly supervised instance segmentation, we are given a set of extreme points annotated training data \mathcal{D} = \{(X_n, Y_n, B_n)\}_{n=1}^{N}. 
%Notation : 
%original image : $\textbf{I}$, cropped image : $\textbf{I}^c$, extreme points in cropped image $ \textbf{e} = \{ (x^{(t)}, y^{(t)})$, $(x^{(l)}, y^{(l)})$, $(x^{(b)}, y^{(b)})$, $(x^{(r)}, y^{(r)}) \}$, 


%좀더 매트하게 적기. 
% \subsection{Preliminary: Extreme Points}
\suha{\subsection{Motivation for Using Extreme Points}
\label{sec:subsection1}}

Extreme points are defined as the outermost points on an object along the cardinal directions: the topmost point $(x^{(t)}, y^{(t)})$, the leftmost point $(x^{(l)}, y^{(l)})$, the bottommost point $(x^{(b)}, y^{(b)})$, rightmost point $(x^{(r)}, y^{(r)})$. Papadopoulos \etal \cite{papadopoulos2017extreme} \suha{have} shown that labeling these points is a more efficient way to bounding box annotation compared to the conventional method of labeling the top-left $(x^{(l)}, y^{(t)})$ and bottom-right $(x^{(r)}, y^{(b)})$ corner points of a box that encompasses the target object. 
\suha{This is because such corner points are hard to be identified as they usually do not belong to the target object area, and thus human annotators often have to adjust their initial corner point labels multiple times.
On the other hand, extreme points can be effortlessly marked and can be converted to a bounding box directly.
Furthermore, extreme points inherently provide more information for the shape and appearance of the target object than corner points since they lie on the object boundary.}




% \subsection{Learning to Generate Pseudo Label from Extreme Points}
\suha{\subsection{Learning Pseudo Label Generator}
\label{sec:subsection2}}

From the geometric characteristics of extreme points, we can deduce the relationship between the target object and the extreme points as follows:
\textbf{First}, each extreme point represents a boundary point in its cardinal direction, which implies that orthogonal to each point within the corresponding bounding box, there exists a foreground point about the target object. 
we will call these set of points as initial foreground point set $ \mathcal{P}_{\textrm{FG}} \in \{ (x^{(t)}, y^{(t)}-\delta)$, $(x^{(l)}+\delta, y^{(l)})$, $(x^{(b)}, y^{(b)}+\delta)$, $(x^{(r)}-\delta, y^{(r)}) \}$.
\textbf{Second}, points outside the bounding box drawn from extreme points are definitive background points, distinct from the target object. we call these set of points as initial background point set $\mathcal{P}_{\textrm{BG}}.$
Based on these premises, the naïve way of utilizing extreme points as weak supervision is using $ \mathcal{P}_{\textrm{FG}} , \mathcal{P}_{\textrm{BG}}$ as point-wise supervision for binary segmentation.

However, the majority of the region within the bounding box remains ambiguous, thereby offering no clear supervisory signal. Consequently,  solely relying on $\mathcal{P}_{\textrm{FG}}$,  $\mathcal{P}_{\textrm{BG}}$ for training is inadequate for predicting a fine-grained object mask.
%Consequently, this approach might underperforms compared to bounding box-based methods that utilize Multiple Instance Learning (MIL) loss. \LHJ{(add ablation study to support this sentence)} 
To provide richer supervision from extreme points for training, we aim to offer additional supervision for the points within the bounding box based on the following assumption:
When propagating points in an image, those within the bounding box that lie on the target object are likely to propagate to $\mathcal{P}_{\textrm{FG}}$ with a high probability, while their probability of propagating to $\mathcal{P}_{\textrm{BG}}$ will be low. 
Similarly, points within the bounding box that lie in the background are expected to propagate to $\mathcal{P}_{\textrm{BG}}$ with a high probability, and to $\mathcal{P}_{\textrm{FG}}$ with a low probability.
Building on this assumption, we select reachable points within the bounding box to leverage them as additional supervision.

% 우리는 image encoder, decoder architecture를 사용한다.
% image encoder 구조는 vision transformer architecture를 사용하는데, 이에 감사하게도, vision transformer의 multi head sefl attention으로 부터 transition probability matrix를 만들었다. 
%MHSA 로부터 Transition probability matrix를 만든 이유는 다음과 같다. 
%1) MHSA is pair-wise affinity contains high-level semantic information 이다. 이는 point를 propagation 시키는데 있어, apprearnce가 비슷하지만 다른 semantic으로 propagation 되는것을 방지해줄수 있다. (low-level image cue like color-pairwise affinity로 이를 만들었다면, Figure 1처럼 pseudo label 만들지 못할것임. 
%2) multi head self attention 은 global feature ependency 를 고려할수 있다. 즉, 이를 통해 만들어진 TPM은 point를 local한 부분으로만 propagation 하도록 제한하지 않는다.
%이는 point propagation이 object가 separated 된 케이스에 대해서도 잘 일어날수 있게 해준다. 

\subsubsection{Constructing Transition Probability Matrix}
\label{sec:subsubsection1}
To propagate points, we construct a Transition Probability Matrix (TPM) from the Multi-Head Self-Attention (MHSA) in the transformer block. 
Specifically, cropped image $I^c \in \mathbb{R}^{H \times W}$ is firstly split into $N$ patches, where each patch is flattened and linearly projected.
These patches serve as the input for a vision transformer $E^{\text{p}}$, where the MHSA in the $i$-th transformer block is denoted as $\mathbf{S}_i \in \mathbb{R}^{N \times N}$. 
We use the 10th transformer block's MHSA $(i=10)$ to balance detail and high-level semantics, as earlier blocks easily miss high-level semantics and later blocks tend to over-smooth patch representation~\cite{Ru_2023_CVPR}.


However, since the queries and keys used to create $\mathbf{S}_i$ are projected from different layers, $\mathbf{S}_i$ is inherently asymmetric. We wish the TPM should be symmetric, meaning that the transition probability from point $p_i$ to point $p_j$ should be equal the probability from point $p_j$ to point $p_i$.
 Given the affinity matrix $\mathbf{S}_i$ from MHSA, we can calculate a symmetric transition probability matrix $\mathbf{T}$ using the following formula,

\begin{equation}\label{eqn:eq2}
    \mathbf{T} = \frac{\mathbf{A} + \mathbf{A}^\top}{2},   \text{  where  } \mathbf{A} = \text{Sinkhorn}(\mathbf{S}_i)
\end{equation}

\noindent where $\text{Sinkhorn}(\cdot)$ refers to the Sinkhorn-Knopp algorithm ~\cite{knight2008sinkhorn}, which is employed to transform a matrix into a doubly-stochastic form.

% Following this, the transition probability matrix \matbhf{T} with $\alpha$ hops can be defined as  
% \begin{equation}\label{eqn:eq2}
%     \mathbf{T} = \mathbf{A}^\alpha
% \end{equation}

\noindent \textbf{Warm-up} Before generating TPM, we warm up the $E^{\text{p}}$ to enhance its ability to differentiate between the background and the target object. Specifically, for the predicted mask probability map $\mathcal{M'}$ obtained through ViT Encoder $E^{\text{p}}$ and auxiliary decoder  $D^{\text{auc}}$, we employ the Multiple Instance Learning (MIL) loss as follow :

\begin{equation}
\label{eq:mil_loss}
\begin{aligned}
\mathcal{L}_{\text{mil}} = \mathcal{L}_{\text{dice}}(&\max_{x}(\mathcal{M}'), \max_{x}(\mathcal{M}_{\text{box}})) \\
&+ \mathcal{L}_{\text{dice}}(\max_y(\mathcal{M}'), \max_y(\mathcal{M}_{\text{box}}))
\end{aligned}
\end{equation}

\noindent where $\max_{x}, \max_y$ indicate max operation along x, y axis, and $\mathcal{L}_{\text{dice}}$ indicates dice loss~\cite{sudre2017generalised}. $\mathcal{M}_{\text{box}} \in \{0,1\}^{H\times W}$ indicates box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise. Note that $D^{\text{auc}}$ is only used for warm-up.

\noindent \textbf{Why TPM from MHSA?}  The extraction of a TPM from the MHSA is beneficial for several reasons. MHSA captures pairwise affinity that contains high-level semantic information. This helps to prevent points from being propagated to other points with a similar appearance but different semantics.
Additionally, MHSA reflects a matrix embodying global feature dependencies, enabling the TPM constructed through it to facilitate point propagation beyond local areas. This allows for the propagation of points across separated segments of an object.

\subsubsection{Point selection algorithm}
\label{sec:subsubsection2}

% Probability FG = average 
 % probability BG = average
 % probdifference 에 기반해서 point i 의 pseudo label 부여

% Let us denote the set of points within the bounding box that can be drawn from extreme point as $\mathcal{P}_{\text{Box}}$. 
% Our objective is to assign pseudo label of points $i \in \mathcal{P}_{\text{Box}}$ based on their tendency of propagation 
% to the foreground points set $\mathcal{P}_{\text{FG}}$ and background point set $\mathcal{P}_{\text{BG}}$.

% We define the tendency of point $i$ to propagate to$\mathcal{P}_{\text{FG}}$ as the average probability among points $j \in \mathcal{P}_{\text{FG}}$
    
Let's denote the set of points within the bounding box that can be drawn from the extreme point as $\mathcal{P}_{\text{Box}}$. Our goal is to estimate the label of points $p_i \in \mathcal{P}_{\text{Box}}$ based on their tendency to propagate towards the foreground points set $\mathcal{P}_{\text{FG}}$ and the background point set $\mathcal{P}_{\text{BG}}$.

We define the probability score for point $p_i$ to propagate towards $\mathcal{P}_{\text{FG}}$ as the average probability of its propagation to each of the four foreground points :

\begin{equation}
\pi_i^{\text{f}}
 = \frac{1}{|\mathcal{P}_{\text{FG}}|} \sum_{p_j \in \mathcal{P}_{\text{FG}}} \mathbf{T}^\alpha(i, j)
\end{equation}

\noindent where $\mathbf{T}^\alpha(i, j)$ represents the transition probability that point 
$p_i$ will propagate to point $p_j$ through $\alpha$ iterations.

Similarly, we define the probability score for point \(p_i \) to propagate towards \( \mathcal{P}_{\text{BG}} \) in an analogous manner. The score is computed as the average probability of point \( p_i \)'s propagation to each of the background points:

\begin{equation}
\pi_i^{\text{b}}
 = \frac{1}{|\mathcal{P}_{\text{BG}}|} \sum_{p_k \in \mathcal{P}_{\text{BG}}} \mathbf{T}^\alpha(i, k)
\end{equation}

Based on the probability scores to $\mathcal{P}_{\text{FG}}$ and $\mathcal{P}_{\text{BG}}$, we can estimate the label for point $p_i \in \mathcal{P}_{\text{Box}}$ using following equation:

\begin{equation}
\hat{y}_i =
\begin{cases}
\mathsf{1}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \geq \tau_{fg} \\
\mathsf{0}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \leq \tau_{bg} \\
\text{unlabeled}, & \text{otherwise}
\end{cases}
\end{equation}

\noindent where $\mathsf{1}$ indicates foreground label and $\mathsf{0}$ indicates background label, and $\tau_{fg}, \tau_{bg}$ are the hyperparameters used to filter out ambiguous points.

\noindent \textbf{Point drop out}
To enhance diversity and prevent overfitting, we adopt a point drop out strategy as an augmentation technique. Within each epoch, for the set of labeled points in bounding box, $p_i \in \mathcal{P}_{\text{Box}}$, we randomly drop $n\%$ of the points and do not use them as supervision. This selective drop-out is applied separately to the foreground-labeled point and background-labeled point sets, ensuring that maintains a dynamic and balanced representation throughout the learning process.



\subsubsection{Training Objective}
\label{sec:subsubsection3}


% \LHJ{HJ : explain example sample of MIL adopted sample, should I explain about masking strategy for unlabeled point region?} 
\noindent \textbf{Point Loss}
We construct binary mask $\mathcal{\hat{Y}}$ using set of points $\mathcal{P}_{\text{FG}} \cup \mathcal{P}_{\text{BG}} \cup \mathcal{P}_{\text{labeled}}$, where $\mathcal{P}_{\text{labeled}} = \{ p_i \mid p_i \in \mathcal{P}_{\text{Box}}, \hat{y}_i \neq \text{unlabeled} \} $.
We use dice loss between $\mathcal{\hat{Y}}$ between predicted mask probability $\mathcal{M}^{s}$ for the point loss. However, there are cases where points cannot be selected using the point selection algorithm ($ | \mathcal{P}_{\text{labeled}} | = 0 $).  For these samples, we applied an additional MIL loss used in Eq ~\ref{eq:mil_loss}.
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{point}} =  \mathcal{L}_{\text{dice}}(\mathcal{M}^{s},\mathcal{\hat{Y}}) + \mathds{1}_{\{|\mathcal{P}_{\text{labeled}}| = 0\}} \lambda_{mil} \mathcal{L}_{\text{mil}}
\end{aligned}
\end{equation}

\noindent where $\mathds{1}$ is indicator function. 
Note that samples subjected MIL loss account for only about $7\%$ of the entire sample, so EXITS does not heavily depend on MIL loss.

\noindent \textbf{Conditional Random Field Loss} 
To further refine the predicted mask, we employ CRF loss~\cite{crf} within an online teacher-student manner as in ~\cite{Lan_2023_CVPR}. We first calculate the average mask prediction $\mathcal{M}^{\text{avg}}$ produced by the student network and teacher network, denoted as $\mathcal{M}^{\text{avg}}$ = $(\mathcal{M}^{s} 
 + \mathcal{M}^{t}) / 2$  . The averaged mask is then refined through the mean-field algorithm and subsequently utilized as a pseudo ground-truth mask $\mathcal{M}^{\text{refine}}$. This approach enables the network to progressively yield a more detailed object mask.
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{crf}} = \mathcal{L}_{\text{dice}}(\mathcal{M}^{s},\mathcal{M}^{\text{refine}})
\end{aligned}
\end{equation}

\noindent Formally, the overall loss function of EXITS can be formulated as :
\begin{equation}
\begin{aligned}
\mathcal{L}_{overall} =  \lambda_{point} \mathcal{L}_{\text{point}} +  \lambda_{crf} \mathcal{L}_{\text{crf}} 
\end{aligned}
\end{equation}

\iftrue
\LHJ{
\subsection{Learning a Fully Supervised Model}
\label{sec:subsection3}

In the second stage, EXITS employs the trained pseudo label generator to create pseudo mask labels that serve as ground-truth labels for training a fully supervised instance segmentation model. 
To generate the pseudo mask labels, images containing $k$ instances are cropped around the corresponding extreme point annotations. These $k$ cropped images are then fed into the trained pseudo labeler, yielding a pseudo mask for each extreme point annotation. 
The decoupled design of the instance segmentation and pseudo labeling models allows for our pseudo labels to be seamlessly integrated into any fully supervised instance segmentation model, unlike other approaches~\cite{lan2021discobox,tian2021boxinst, li2022box,li2023sim, cheng2023boxteacher}.

}
% \fi

% \hsh{\subsection{Learning a fully supervised model}
% \label{sec:subsection3_1}
% In the second stage, EXITS employs the trained \LHJ{pseudo label} generator to create pseudo mask labels, which are then used to train a fully supervised instance segmentation model.
% To generate pseudo mask labels, images containing multiple objects are cropped around each object to match the input format of the pseudo label generator. This process results in the generation of object-wise pseudo mask labels.
% Subsequently, these object-wise masks are combined according to the cropped regions to form the final pseudo mask labels.
% These pseudo mask labels can be applied to train any instance segmentation framework. 
% In our study, we apply SOLOv2~\cite{wang2020solov2} and Mask2Former~\cite{cheng2022masked} to demonstrate the generality and effectiveness of our approach.}


%Typically, in a fully supervised instance segmentation setting, a set of annotated training data is required, denoted as \( \mathcal{D} = \{ (X_n, C_n, B_n, M_n) \}_{n=1}^{N} \), where \( N \) is the number of images, \( C_n = \{c_n^k\}_{k=1}^{K} \), \( B_n = \{b_n^k\}_{k=1}^{K} \), and \( M_n = \{m_n^k\}_{k=1}^{K} \) denote the class-level, box-level, and pixel-level annotations, respectively, with \( K \) representing the number of instances in the image \( X_n \). 

% With given extreme point annotation \( E_n = \{e_n^k\}_{k=1}^{K} \), \( B_n \) can be obtained directly by reformatting $E_n$, and \( M_n \) is substituted by a pseudo mask \( \hat{M}_n \), generated by inputting the cropped region around the corresponding extreme point annotation into a pseudo-labeler. Thanks to separated framework, our pseudo labels can be effortlessly incorporated into any fully supervised instance segmentation model, unlike other approaches~\cite{lan2021discobox,tian2021boxinst, li2022box,li2023sim, cheng2023boxteacher}.

%필요한 수식들 정리해놓기. 

==> sections/03_method_backup_231117.tex <==
\section{Proposed Method}

%Feedback : Stage 1 인거 명시적으로 설명해주기. 
\begin{figure*}[t]
    \centering
        \includegraphics[width=\textwidth]{figures/overall_pipeline_v2.7.pdf}
        \caption{\textbf{Overview of the first stage of EXITS framework.}
                The pseudo label generator is trained on images cropped around each object using the extreme points, aiming to predict binary masks.
                Training leverages two loss functions: $\mathcal{L}_\text{crf}$ aligns images before and after CRF~\cite{crf} processing,
                % $\mathcal{L}_\text{mil}$ ensures a foreground predicted pixel exists in every row and column of the bounding box,
                and $\mathcal{L}_\text{point}$ uses extreme points-derived pseudo point labels for precise pixel-wise supervision.
                To generate these pseudo point labels, EXITS obtains initial foreground and background points from extreme points, then employs the similarity matrix from warm-up trained similarity extractor for label propagation.
                After propagation, pseudo point labels are produced based on the difference of propagation score from the inital foreground and background points.
                Point dropout is applied as an augmentation generating the final pseudo point labels.}
                % pseudo point labels are initially generated from extreme points, with the self-attention of warm-up trained VIT facilitating label propagation.
                % The resulting pseudo point labels are dynamically dropped out to establish the final set of pseudo point labels.}}
    \label{fig:pipeline}
    \vspace{-3mm}
\end{figure*} 
% Feedback : 왜 pseudo labeler의 output으로는 final model prediction으로 사용할 수 없는지 설명하기. 
% Feedback : stage 2 instance segmentation model이랑 stage 1 instance segmentation model을 "명시적으로"분리해서 설명하기
\iffalse
    Our approach to weakly supervised instance segmentation is divided into two stages: (1) Generating pixel-wise segmentation labels of each object annotated by extreme points, and (2) Learning DNN for instance segmentation with the generated pseudo labels by the first stage. 
    In the first stage, the segmentation model receives images that have been cropped around objects annotated by extreme points \suhac{}. It is then trained to predict the corresponding object mask supervised by reachable points from extreme points and background points as~\Fig{pipeline}. 
    In the second stage, we can apply any fully supervised instance segmentation pipeline~\cite{wang2020solov2, cheng2022masked} using pseudo label generated by the first stage. Therefore, we will focus on describing the first stage. 
    
    The remainder of this section describes the preliminary of extreme points (Sec.~\ref{sec:subsection2}), and how to train the segmentation model to generate object masks from corresponding extreme points (Sec.~\ref{sec:subsection4}, Sec.~\ref{sec:subsection5}). 
\fi


\suha{EXITS consists of two stages: (1) learning a model that generates pseudo segmentation labels of training images using their extreme point labels, and (2) training an instance segmentation model using the pseudo labels.
 
In the first stage, an object image cropped around each object using extreme points is used as an input to the pseudo label generator so that the model learns to predict a binary mask of the object within the cropped image.
 On the other hand, the instance segmentation model in the second stage, which is our target model, learns to detect and segment multiple objects. 
Note that the pseudo label generator deals with an easier task, \ie, instance segmentation on a single object image, which enables to improve the quality of pseudo labels it generates.
The entire pipeline of EXITS is illustrated in~\Fig{stage}.

Since the second stage is the conventional supervised learning that can be applied to any instance segmentation model, this section elaborates mostly on the first stage, in particular, how EXITS provides the pseudo label generator with effective supervision for segmentation. 
The overall pipeline of the first stage is illustrated in Fig.~\ref{fig:pipeline}.
The key idea of EXITS is to retrieve pixels likely to belong to the object given the extreme points, and exploit them as (sparse) supervision for learning segmentation.
This idea is realized by propagating the extreme points to other pixels within the input object image, while considering the extreme points as a subset of true pixels of the object.

The remainder of this section first discusses extreme points and advantages of using them (\Sec{subsection1}), and then presents details of the first stage (\Sec{subsection2}) and the second stage (\Sec{subsection3}) of EXITS.
% and then presents details of point supervision generation and loss functions for learning the pseudo label generator (\Sec{subsection2}).}
% \LHJ{Lastly, we describe how the pseudo labels from first stage are integrated into existing fully supervised instance segmentation models in the second stage. (\Sec{subsection3})
}
% \hsh{
% The EXtreme point-based InsTance Segmentation (EXITS) framework operates through two stages: (1) It learns to create pixel-wise segmentation pseudo labels for training images, guided by their extreme point labels.
% (2) It employs these pseudo labels to train a fully supervised instance segmentation model.
% Since any conventional instance segmentation model can be utilized in the second stage, we focus on describing the first stage -- generating a precise pseudo segmentation label given extreme points.

% In the first stage, the input image is cropped around each object using extreme points, and the model is trained to predict a binary mask of the input object of interest.
% Since pixel-wise segmentation labels are inaccessible, EXITS proposes to propagate foreground labels from the extreme points, and background labels from the pixels located outside of the object of interest.
% \Fig{pipeline} describes the overall pipeline of the first stage.
% The remainder of this section describes the preliminary of extreme points (\Sec{subsection2}), the pipeline of generating pseudo mask labels (\Sec{subsection4}), and our objective functions (\Sec{subsection5}).}


%In the setting of weakly supervised instance segmentation, we are given a set of extreme points annotated training data \mathcal{D} = \{(X_n, Y_n, B_n)\}_{n=1}^{N}. 
%Notation : 
%original image : $\textbf{I}$, cropped image : $\textbf{I}^c$, extreme points in cropped image $ \textbf{e} = \{ (x^{(t)}, y^{(t)})$, $(x^{(l)}, y^{(l)})$, $(x^{(b)}, y^{(b)})$, $(x^{(r)}, y^{(r)}) \}$, 


%좀더 매트하게 적기. 
% \subsection{Preliminary: Extreme Points}
\suha{\subsection{Motivation for Using Extreme Points}
\label{sec:subsection1}}

Extreme points are defined as the outermost pixels on an object along the cardinal directions: the topmost point $(x^{(t)}, y^{(t)})$, the leftmost point $(x^{(l)}, y^{(l)})$, the bottommost point $(x^{(b)}, y^{(b)})$, rightmost point $(x^{(r)}, y^{(r)})$. Papadopoulos \etal \cite{papadopoulos2017extreme} \suha{have} shown that labeling these points is a more efficient way to bounding box annotation compared to the conventional method of labeling the top-left $(x^{(l)}, y^{(t)})$ and bottom-right $(x^{(r)}, y^{(b)})$ corner points of a box that encompasses the target object. 
\suha{This is because such corner points are hard to be identified as they usually do not belong to the target object area, and thus human annotators often have to adjust their initial corner point labels multiple times.
On the other hand, extreme points can be effortlessly marked and can be converted to a bounding box directly.
Furthermore, extreme points inherently provide more information for the shape and appearance of the target object than corner points since they lie on the object boundary.}



\suha{\subsection{Learning Pseudo Label Generator}
\label{sec:subsection2}}
\iffalse
    \LHJ{Our pseudo label generator consists of student network image encoder $E$ and mask decoder $D$ and encoder for TPM $E_{tpm}$}
    From the geometric properties of extreme points, we deduce the following relationships between an object and its extreme points.
    First, each extreme point represents a boundary point of the object along its cardinal direction. This indicates that foreground points are likely to exist in a direction perpendicular to the bounding box from each extreme point. 
    we consider these points as initial foreground point set $ \mathcal{P}_{\textrm{FG}} = \{ (x^{(t)}, y^{(t)}-\delta)$, $(x^{(l)}+\delta, y^{(l)})$, $(x^{(b)}, y^{(b)}+\delta)$, $(x^{(r)}-\delta, y^{(r)}) \}$.
    Second, points outside the bounding box defined by the extreme points are definitive background points, distinct from the target object. we consider these points as initial background point set $\mathcal{P}_{\textrm{BG}} := \{ (x,y) | \textrm{max}(x-x^{(r)}, x^{(l)}-x, y-y^{(b)}) > 0, y^{(t)}-y \}.$
    
    A naïve way of utilizing extreme points as weak supervision is using $ \mathcal{P}_{\textrm{FG}}$ and $\mathcal{P}_{\textrm{BG}}$ as point-wise supervision for binary segmentation.
    However, in this approach, most of the region within the bounding box remains unlabeled, thereby offering no supervisory signal. Consequently, $\mathcal{P}_{\textrm{FG}}$ and $\mathcal{P}_{\textrm{BG}}$ are insufficient for learning crisp object masks. 
    To generate richer supervision from extreme points, we aim to offer additional supervision for the points within the bounding box based on the following assumption:
    \LHJmodified{
    If we diffuse points in a bounding box by a random walk~\cite{lovasz1993random}, guided by a transition probability matrix constructed based on semantic similarity between points, points that lie on the target object are likely to propagate to $\mathcal{P}_{\textrm{FG}}$ with a high probability, while their probability of propagating to $\mathcal{P}_{\textrm{BG}}$ will be low. Similarly, points lie in the background are expected to propagate to $\mathcal{P}_{\textrm{BG}}$ with a high probability, and to $\mathcal{P}_{\textrm{FG}}$ with a low probability. 
    }
    Building on this assumption, we estimate labels of points within the bounding box and leverage them as additional supervision to train pseudo label generator.
\fi

The pseudo label generator aims to predict a binary mask of an object given an image cropped around it.
The generator consists of ViT encoder and mask decoder.
We retrieve points that likely belong to the object (foreground) or the background to train the generator using an initial set of labels deduced from extreme points.
An initial set of foreground points is extreme points, denoted as $\mathcal{P}_{\textrm{FG}}:= \big\{ (x^{(t)}, y^{(t)}-\delta), (x^{(l)}+\delta, y^{(l)}), (x^{(b)}, y^{(b)}+\delta), (x^{(r)}-\delta, y^{(r)}) \big\}$, where $\delta$ is a margin that pushes these points toward the center of an object to avoid points on the boundary.
On the other hand, the initial set of background points $\mathcal{P}_{\textrm{BG}}$ consists of the points located outside the bounding box defined by the extreme points.
% To provide supervision for the set of unlabeled points denoted as $P_\textrm{U}:= \big\{ (x,y) | (x,y) \notin \mathcal{P}_{\textrm{FG}} \cup \mathcal{P}_{\textrm{BG}}\big\}$, we measure the semantic similarity of these points to members of $\mathcal{P}_{\textrm{FG}}$ and $\mathcal{P}_{\textrm{BG}}$.
To assign pseudo point labels for unlabeled points within the bounding box denoted as $\mathcal{P}_{\textrm{Box}}$, the initial labels from $\mathcal{P}_{\textrm{FG}}$ and $\mathcal{P}_{\textrm{BG}}$ are propagated to $\mathcal{P}_{\textrm{Box}}$ based on the semantic similarity of these points.
% we measure the semantic similarity of these points to members of $\mathcal{P}_{\textrm{FG}}$ and $\mathcal{P}_{\textrm{BG}}$.
Points that are likely to be propagated to the members of $\mathcal{P}_{\textrm{FG}}$ but not to those of $\mathcal{P}_{\textrm{BG}}$ are classified as pseudo foreground points.
Conversely, points that are more likely to be propagated to the members of $\mathcal{P}_{\textrm{BG}}$ than to $\mathcal{P}_{\textrm{FG}}$ are classified as pseudo background points.

\subsubsection{Constructing Transition Probability Matrix}
\label{sec:subsubsection1}
\iffalse
    To propagate points, we construct a transition probability matrix (TPM) from the multi-head self-attention (MHSA) in a pretrained transformer block. 
    Specifically, a cropped image $I^c \in \mathbb{R}^{H \times W}$ is firstly split into $N \times N$ patches, where each patch is flattened and linearly projected.
    These patches serve as the input for a pre-trained vision transformer $E^{\text{p}}$, and we adopt a self-attention matrix in the $i$-th transformer block's MHSA, which is denoted as $\mathbf{S}_i \in \mathbb{R}^{N \times N \times N \times N}$. 
    Note that $\mathbf{S}_i$ is inherently asymmetric since the queries and keys used to create $\mathbf{S}_i$ are projected from different layers. We wish the TPM should be symmetric, meaning that the transition probability from point $p_i$ to point $p_j$ should be equal the probability from point $p_j$ to point $p_i$.
     Given the self-attention matrix $\mathbf{S}_i$ from the MHSA, a symmetric transition probability matrix $\mathbf{T}$ is calculated by
    \begin{equation}\label{eqn:eq2}
        \mathbf{T} = \frac{\mathbf{A} + \mathbf{A}^\top}{2},   \text{  where  } \mathbf{A} = \text{Sinkhorn}(\mathbf{S}_i)
    \end{equation}
    
    \noindent and $\text{Sinkhorn}(\cdot)$ refers to the Sinkhorn-Knopp algorithm ~\cite{knight2008sinkhorn}, which transforms a matrix into a doubly-stochastic form.
    
    \noindent \textbf{Warm-up.} Before generating $\mathbf{T}$, we warm up the vision transformer to enhance its ability to differentiate between the background and the target object. Specifically, for the predicted mask probability map $\mathcal{M'}$ obtained through ViT Encoder $E^{\text{p}}$ and auxiliary decoder $D^{\text{auc}}$, we employ a multiple instance learning (MIL) loss as follow:
    
    \begin{equation}
    \label{eq:mil_loss}
    \begin{aligned}
    \mathcal{L}_{\text{mil}} = \mathcal{L}_{\text{dice}}\big(&\max_{x}(\mathbf{M}), \max_{x}(\hat{\mathbf{Y}}_\text{box})\big) \\
    &+ \mathcal{L}_{\text{dice}}\big( \max_y(\mathbf{M}), \max_y(\hat{\mathbf{Y}}_\text{box}) \big)
    \end{aligned}
    \end{equation}
    
    \noindent where $\max_{x}, \max_y$ indicate max operation along $x$, $y$ axes, respectively, and $\mathcal{L}_{\text{dice}}$ indicates the dice loss~\cite{sudre2017generalised}. $\hat{\mathbf{Y}}_\text{box} \in \{0,1\}^{H\times W}$ indicates box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise. Note that $D^{\text{auc}}$ is only used for warm-up.
    
    \noindent \textbf{Why TPM from MHSA?}  The extraction of a TPM from the MHSA is beneficial for several reasons. The MHSA captures pairwise affinity between patches based on high-level semantic information. This helps to prevent points from being propagated to other points with a similar appearance but different semantics.
    Additionally, the MHSA reflects a matrix embodying global feature dependencies, enabling the TPM constructed through it to facilitate point propagation beyond local areas. In particular, this allows to propagate points across separated segments of an object.
\fi
\noindent \textbf{Training similarity extractor.}
To capture the semantic similarity between points, EXITS leverages an attention matrix obtained from a Multi-Head Self-Attention (MHSA) in vision transformer (ViT).
% Since initial ViT is not capable of distinguishing between foreground and background, the similarity extractor is trained for several epochs with Multiple Instance Learning (MIL) loss~\cite{hsu2019weakly, tian2021boxinst} as a warm-up training.
%Since initial ViT is not capable of distinguishing between foreground and background
Since the attention matrix from initial ViT is not capable of capturing the difference between foreground and background, we train an extra ViT encoder called \textit{similarity extractor}, which is trained for several epochs with Multiple Instance Learning (MIL) loss~\cite{hsu2019weakly, tian2021boxinst}.
% The MIL loss trains the segmentation model using ground-truth bounding boxes.
% Since extreme points already encompass the bounding box information, our method is also capable of utilizing it.
% The MIL loss enables the training of a segmentation model using only bounding box labels.
% Since extreme points already contain bounding box information, our method is also capable of utilizing it.
% Specifically, for the predicted mask probability map $\mathbf{M}$, we employ the MIL loss as follows:
% \begin{equation}
%     \label{eq:mil_loss}
%     \begin{aligned}
%         \mathcal{L}_{\text{mil}} = \mathcal{L}_{\text{dice}}\big(&\max_{x}(\mathbf{M}), \max_{x}(\hat{\mathbf{Y}}_\text{box})\big) \\
%         &+ \mathcal{L}_{\text{dice}}\big( \max_y(\mathbf{M}), \max_y(\hat{\mathbf{Y}}_\text{box}) \big) \;,
%     \end{aligned}
% \end{equation}
% where $\max_{x}, \max_y$ indicate max operation along $x$, $y$ axes, respectively, and $\mathcal{L}_{\text{dice}}$ indicates the dice loss~\cite{sudre2017generalised}. $\hat{\mathbf{Y}}_\text{box} \in \{0,1\}^{H\times W}$ indicates a box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise.
% Specifically, MIL loss is implemented by calculating the discrepancy between the projection of the mask prediction $\mathbf{M}$ and the mask from bounding box $\hat{\mathbf{Y}}_\text{box}$, which is defined as
Specifically, MIL loss calculates the discrepancy between the projection of the prediction $\mathbf{M}$ and the projection of bounding box mask $\hat{\mathbf{Y}}_\text{box} \in \{0,1\}^{H\times W}$ generated by assigning 1 to the locations in the ground-truth box and 0 otherwise.
Formally, the MIL loss is defined as
% $\hat{\mathbf{Y}}_\text{box} \in \{0,1\}^{H\times W}$ indicates a box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise.
\begin{equation}
    \label{eq:mil_loss}
    \begin{aligned}
        \mathcal{L}_{\text{mil}} = \mathcal{L}_{\text{dice}}\big(&\text{Proj}_{x}(\mathbf{M}), \text{Proj}_{x}(\hat{\mathbf{Y}}_\text{box})\big) \\
        &+ \mathcal{L}_{\text{dice}}\big( \text{Proj}_y(\mathbf{M}), \text{Proj}_y(\hat{\mathbf{Y}}_\text{box}) \big) \;,
    \end{aligned}
\end{equation}
where $\mathcal{L}_{\text{dice}}$ is the dice loss~\cite{sudre2017generalised}, and $\text{Proj}_x: \mathbb{R}^{H\times W} \mapsto \mathbb{R}^{W}$ and $\text{Proj}_y: \mathbb{R}^{H\times W} \mapsto \mathbb{R}^{H}$ are projection operations that apply max operation across each column and each row vector of the input matrix, respectively.
% $\hat{\mathbf{Y}}_\text{box} \in \{0,1\}^{H\times W}$ indicates a box-shaped mask generated by assigning 1 to the locations in the ground-truth box and 0 otherwise.
% After the warm-up training, the similarity extractor is frozen without further updates.
The similarity extractor is frozen without further updates during the training of the pseudo label generator.

% To measure the semantic similarity between points, EXITS treats each point as a node in a fully connected graph and utilizes the transition probability between these nodes as their semantic similarity.
We treat each point as a node in a fully connected graph and construct the transition probability between these nodes using their semantic similarity.
To compute the transition probability matrix, a cropped image is divided into $N \times N$ patches and flattened, then fed into the similarity extractor.
The similarity matrix $\mathbf{S} \in \mathbb{R}^{N^2 \times N^2}$ is then derived by averaging the self-attention matrices from multiple attention heads of the $i$-th transformer blocks.
To construct transition probability matrix $\mathbf{T}$ a doubly stochastic form, the Sinkhorn Normalization is applied to $\mathbf{S}$, which is calculated by
\begin{equation}\label{eqn:eq2}
    \mathbf{T} = \frac{\mathbf{A} + \mathbf{A}^\top}{2},   \text{  where  } \mathbf{A} = \text{Sinkhorn}(\mathbf{S}) \;,
\end{equation}
where $\text{Sinkhorn}(\cdot)$ is the Sinkhorn-Knopp algorithm ~\cite{knight2008sinkhorn}.

The extraction of the transition probability matrix from the MHSA mechanism offers two advantages.
Firstly, since the MHSA captures high-level semantic relationships between points, the resulting transition probability matrix prevents points from being propagated to other points with a similar appearance but different semantics.
Secondly, the MHSA calculates similarities for all pairings between points, thereby yielding a transition probability matrix for a fully connected graph.
This allows the propagation of labels across separated segments of an object, enhancing the accuracy of the label assignment process.

% \iffalse
\subsubsection{Retrieving Pseudo Point Supervision}
\label{sec:subsubsection2}
% Our goal is to predict the labels of points $\mathbf{p}_i \in \mathcal{P}_{\text{Box}}$ \todo{based on their tendency to propagate towards the foreground points set $\mathcal{P}_{\text{FG}}$ and the background point set $\mathcal{P}_{\text{BG}}$.}
% Our goal is to predict the labels of points $\mathbf{p}_i \in \mathcal{P}_{\text{Box}}$ \todo{based on their tendency to propagate towards the foreground points set $\mathcal{P}_{\text{FG}}$ and the background point set $\mathcal{P}_{\text{BG}}$.}
A pseudo point label of $\mathbf{p}_i \in \mathcal{P}_{\text{Box}}$ is assigned by its propagation score calculated with transition probability from each member of $\mathcal{P}_{\text{FG}}$ and $\mathcal{P}_{\text{BG}}$ to $\mathbf{p}_i$.
We define a foreground propagation score $\pi_i^{\text{(f)}}$ of $\mathbf{p}_i$ as
% The propagation score $\pi_i^{\text{(f)}}$ for point $\mathbf{p}_i$ to propagate to the members of $\mathcal{P}_{\text{FG}}$ is the average probability of its propagation to each of the four foreground points:
\begin{equation}
    \pi_i^{\text{(f)}}
     = \frac{1}{|\mathcal{P}_{\text{FG}}|} \sum_{\mathbf{p}_j \in \mathcal{P}_{\text{FG}}} \mathbf{T}^\alpha(j, i) \;,
    \end{equation}
\noindent where $\mathbf{T}^\alpha(j, i)$ denotes the transition probability that point $\mathbf{p}_j$ propagate to point $\mathbf{p}_i$ through $\alpha$ hops.
Similarly, we define a background propagation score of $\mathbf{p}_i$ in an analogous manner, denoted as
\begin{equation}
    \pi_i^{\text{(b)}}
     = \frac{1}{|\mathcal{P}_{\text{BG}}|} \sum_{\mathbf{p}_k \in \mathcal{P}_{\text{BG}}} \mathbf{T}^\alpha(k, i) \;.
\end{equation}
% Using these scores, the pseudo label $\hat{l}_i$ of $\mathbf{p}_i$ is defined as follows:
% \begin{equation}
%     \hat{l}_i =
%         \begin{cases}
%             \mathsf{1}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \geq \tau_{\text{FG}} \\
%             \mathsf{0}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \leq \tau_{\text{BG}} \\
%             \text{unlabeled}, & \text{otherwise} \;,
%         \end{cases}
% \end{equation}
Using these scores, the set of pseudo foreground points $\hat{\mathcal{P}}_{\text{FG}}$ is defined as
\begin{equation}
    % \mathcal{D}_\text{s} := \big\{ (s, \{c\}): \exists (s,Y) \in \mathcal{D}, \, |Y| = 1, \, c \in Y  \big\} \;.
    \hat{\mathcal{P}}_\text{FG} := \big\{ (x_i, y_i): \exists (x_i, y_i) \in \mathcal{P}_\text{Box}, \, \pi_i^{\text{(f)}}-\pi_i^{\text{(b)}} \geq \tau_{\text{FG}} \big\} \;,
\end{equation}
where $\tau_\text{FG}$ is the threshold hyperparameter.
Similarly, the set of pseudo background points $\hat{\mathcal{P}}_\text{BG}$ is defined as
\begin{equation}
    % \mathcal{D}_\text{s} := \big\{ (s, \{c\}): \exists (s,Y) \in \mathcal{D}, \, |Y| = 1, \, c \in Y  \big\} \;.
    \hat{\mathcal{P}}_\text{BG} := \big\{ (x_i, y_i): \exists (x_i, y_i) \in \mathcal{P}_\text{Box}, \, \pi_i^{\text{(f)}}-\pi_i^{\text{(b)}} \leq \tau_{\text{BG}} \big\} \;,
\end{equation}
where $\tau_\text{BG}$ is the threshold hyperparameter.
% where $\mathsf{1}$ indicates foreground label and $\mathsf{0}$ indicates background label, and $\tau_{\text{FG}}, \tau_{\text{BG}}$ are the hyperparameters used to filter out ambiguous points.

\noindent \textbf{Point dropout.}
To enhance the diversity of the pseudo point supervision and prevent overfitting, we adopt an augmentation technique called \textit{point dropout}.
% Let $\hat{\mathcal{P}}_\text{FG}$, $\hat{\mathcal{P}}_\text{BG}$ denote foreground-labeled point set and background-labeled point set in bounding box, respectively.
% For each epoch, point dropout removes a random subset of $\hat{\mathcal{P}}_\text{FG}$ and $\hat{\mathcal{P}}_\text{BG}$ independently, and the removed subset are not used for the training in the epoch.
For each epoch, point dropout independently eliminates a random subset from both $\hat{\mathcal{P}}_\text{FG}$ and $\hat{\mathcal{P}}_\text{BG}$, and the removed subsets are excluded from the training process during that epoch.
% \fi

\iffalse
    \hsh{\subsubsection{Retrieving pseudo point Supervision}
    \label{sec:subsubsection2}
    Our goal is to predict the labels of points $p_i \in \mathcal{P}_{\text{U}}$ based on their tendency to propagate towards $\mathcal{P}_{\text{FG}}$ and $\mathcal{P}_{\text{BG}}$.
    The probability score for point $p_i$ to propagate towards $\mathcal{P}_{\text{FG}}$ is defined as the average probability of its propagation to each of the four foreground points:
    
    \begin{equation}
    \pi_i^{\text{f}}
     = \frac{1}{|\mathcal{P}_{\text{FG}}|} \sum_{p_j \in \mathcal{P}_{\text{FG}}} \mathbf{T}^\alpha(i, j)
    \end{equation}
    
    \noindent where $\mathbf{T}^\alpha(i, j)$ represents the transition probability that point 
    $p_i$ propagate to point $p_j$ through $\alpha$ iterations.
    
    Similarly, we define the probability score for point \(p_i \) to propagate towards \( \mathcal{P}_{\text{BG}} \) in an analogous manner. The score is computed as the average probability of point \( p_i \)'s propagation to each of the background points:
    
    \begin{equation}
    \pi_i^{\text{b}}
     = \frac{1}{|\mathcal{P}_{\text{BG}}|} \sum_{p_k \in \mathcal{P}_{\text{BG}}} \mathbf{T}^\alpha(i, k)
    \end{equation}
    
    Our method estimates the label $\hat{l}_i$ for a point $p_i \in \mathcal{P}_{\text{Box}}$, based on the $\pi_i^{\text{f}}$ and $\pi_i^{\text{b}}$ as follows:
    
    \begin{equation}
    \hat{l}_i =
    \begin{cases}
    \mathsf{1}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \geq \tau_{\text{FG}} \\
    \mathsf{0}, & \text{if } \pi_i^{\text{f}} - \pi_i^{\text{b}} \leq \tau_{\text{BG}} \\
    \text{unlabeled}, & \text{otherwise}
    \end{cases}
    \end{equation}
    
    \noindent where $\mathsf{1}$ indicates foreground label and $\mathsf{0}$ indicates background label, and $\tau_{\text{FG}}, \tau_{\text{BG}}$ are the hyperparameters used to filter out ambiguous points.
    
    \noindent \textbf{Point drop-out.}
    \LHJ{
    To enhance diversity \LHJmodified{(of what?)} and prevent overfitting, we adopt a point drop out strategy as an augmentation technique. 
    Let $\hat{\mathcal{P}}_\text{FG}$, $\hat{\mathcal{P}}_\text{BG}$  denote foreground-labeled point set and background-labeled point set in bounding box, respectively. Within each epoch, we randomly drop a subset of the points from $\mathcal{P}_{\text{FG\_Box}}$ and  $\mathcal{P}_{\text{BG\_Box}}$ independently, and do not use them for training.}}
\fi

\subsubsection{Training Objective}
\label{sec:subsubsection3}
% \LHJ{HJ : explain example sample of MIL adopted sample, should I explain about masking strategy for unlabeled point region?} 
\noindent \textbf{Point loss.}
\iffalse
    We construct sparse point matrix mask $\hat{\mathbf{Y}} \in $ using set of points $\mathcal{P}_{\text{FG}} \cup \mathcal{P}_{\text{BG}} \cup \mathcal{P}_{\text{labeled}}$, where $\mathcal{P}_{\text{labeled}} = \{ p_i \mid p_i \in \mathcal{P}_{\text{Box}}, \hat{y}_i \neq \text{unlabeled} \} $.
    We use the dice loss between $\hat{\mathbf{Y}}$ and the predicted mask probability $\mathbf{M}$ for the point loss. However, there are cases where points cannot be selected using the point selection algorithm ($ | \mathcal{P}_{\text{labeled}} | = 0 $).  For these samples, we applied the MIL loss used in Eq.(\ref{eq:mil_loss}) additionally.
    \begin{equation}
    \begin{aligned}
    \mathcal{L}_{\text{point}} =  \mathcal{L}_{\text{dice}}(\mathbf{M},\hat{\mathbf{Y}}) + \mathds{1}_{\{|\mathcal{P}_{\text{labeled}}| = 0\}} \lambda_{\text{mil}} \mathcal{L}_{\text{mil}}
    \end{aligned}
    \end{equation}
    \noindent where $\mathds{1}$ is indicator function.
\fi
Let $(x_i, y_i)$ denote the 2D coordinates of point $\mathbf{p}_i$ in label space $\mathbb{R}^{N \times N}$.
We construct sparse binary mask $\hat{\mathbf{Y}}\in \mathbb{R}^{N \times N}$ as follows:
\begin{equation}
    \hat{\mathbf{Y}}(x_i, y_i) = 
        \begin{cases} 
            \mathsf{1} & \text{if } \mathbf{p}_i \in  \mathcal{P}_{\text{FG}} \cup \hat{\mathcal{P}}_\text{FG} \\
            \mathsf{0} & \text{otherwise} \;.% p_i \in  \mathcal{P}_{\text{BG}} \cup \hat{\mathcal{P}}_\text{BG} 
        \end{cases}
\end{equation}

\noindent Furthermore, we construct a masking matrix $ \mathbf{K} \in \mathbb{R}^{N \times N} $, which encodes region with point-supervision as follows:
\begin{equation}
    \mathbf{K}(x_i, y_i) = 
    \begin{cases} 
        \mathsf{1} & \text{if } \mathbf{p}_i \in \mathcal{P}_\text{FG} \cup \hat{\mathcal{P}}_\text{FG} \cup \mathcal{P}_\text{BG} \cup \hat{\mathcal{P}}_\text{BG} \\
        \mathsf{0} & \text{otherwise} \;. % p_i \in  \mathcal{P}_{\text{BG}} \cup \hat{\mathcal{P}}_\text{BG} 
    \end{cases}
\end{equation}

\noindent We employ the dice loss between $\hat{\mathbf{Y}}$ and the predicted mask probability $\mathbf{M}$.
Prior to computing the loss, we perform an element-wise multiplication of $\mathbf{K}$ with $\mathbf{M}$ to guarantee that the loss signal is not applied to regions with unlabeled points.
% However, there are cases where points cannot be selected using the point selection algorithm ($ | \hat{\mathcal{P}}_\text{FG} \cup \hat{\mathcal{P}}_\text{BG} | = 0 $).
% For these cases, we applied the MIL loss in~\Eq{mil_loss} additionally.
In cases where none of the points is retrieved with the point retrieval algorithm, \ie, $ | \hat{\mathcal{P}}_\text{FG} \cup \hat{\mathcal{P}}_\text{BG} | = 0 $, we apply the MIL loss in~\Eq{mil_loss} additionally.
The point loss is defined as:
% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{\text{point}} =
%             &\ \mathcal{L}_{\text{dice}}(\mathbf{M} \odot \mathbf{K},\hat{\mathbf{Y}}) + \\
%             & \mathds{1}_{\{|\hat{\mathcal{P}}_\text{FG} \cup \hat{\mathcal{P}}_\text{BG}| = 0\}} \lambda_{\text{mil}} \, \mathcal{L}_{\text{mil}} \;,
%     \end{aligned}
% \end{equation}
\begin{equation}
        \mathcal{L}_{\text{point}} = \mathcal{L}_{\text{dice}}(\mathbf{M} \odot \mathbf{K},\hat{\mathbf{Y}}) + \mathds{1}_{\{|\hat{\mathcal{P}}_\text{FG} \cup \hat{\mathcal{P}}_\text{BG}| = 0\}} \lambda_{\text{mil}} \, \mathcal{L}_{\text{mil}} \;,
\end{equation}
\noindent where $\odot$ is harmard-product operator, $\mathds{1}$ is indicator function, and $\lambda_{\text{mil}}$ is a balancing hyper-parameter.

\noindent \textbf{Conditional random field loss.} 
% \LHJ{To further refine the predicted mask, we employ the CRF~\cite{crf} in an online teacher-student manner as in~\cite{Lan_2023_CVPR}.
% We first calculate the average mask prediction $\mathbf{M}^{\text{avg}}$ produced by the student network and teacher network, denoted as $\mathbf{M}^{\text{avg}}$ = $(\mathbf{M} + \mathbf{M}^{t}) / 2$.
% To further refine the predicted mask, EXITS employs self-supervised learning loss by generating online pseudo labels by applying the CRF~\cite{crf} to its own prediction in an online teacher-student manner as in~\cite{Lan_2023_CVPR}.
To further refine the predicted mask, EXITS employs CRF loss as in~\cite{Lan_2023_CVPR}.
Specifically, EXITS utilizes a teacher network obtained by the exponential moving average of training network, \ie, ViT encoder and mask decoder in Pseudo labeled generator parameters.
Subsequently, mask predictions from both the training network and the teacher network are averaged to obtain $\mathbf{M}^{\text{avg}}$.
% Specifically, we first calculate the average mask prediction $\mathbf{M}^{\text{avg}}$ produced by the student network and teacher network.
% Then, $\mathbf{M}^{\text{avg}}$ is refined through CRF~\cite{crf} by using the mean-field algorithm~\cite{krahenbuhl2011efficient} and the refined mask $\mathbf{M}^{\text{refine}}$ is utilized as pseudo ground-truth mask using the dice loss as follows:
Then, $\mathbf{M}^{\text{avg}}$ is refined through CRF~\cite{crf} by using the mean-field algorithm~\cite{krahenbuhl2011efficient} and utilized as pseudo ground-truth mask using the dice loss as follows:
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{\text{crf}} = \mathcal{L}_{\text{dice}}(\mathbf{M},\textrm{CRF}(\mathbf{M}^{\text{avg}})) \; ,
    \end{aligned}
\end{equation}
where $\textrm{CRF}(\cdot)$ is the CRF operation.
This approach enables the network to yield a more detailed object mask progressively.

\noindent In summary, the overall loss function of EXITS is
\begin{equation}
\begin{aligned}
\mathcal{L}_{overall} =  \lambda_{\text{point}} \mathcal{L}_{\text{point}} +  \lambda_{\text{crf}} \mathcal{L}_{\text{crf}} \;,
\end{aligned}
\end{equation}
where $\lambda_{\text{point}}$ and $\lambda_{\text{crf}}$ are balancing hyper-parameters.

\subsection{Learning a Fully Supervised Model}
\label{sec:subsection3}

In the second stage, EXITS employs the trained pseudo label generator to create pseudo mask labels that serve as ground-truth labels for training a fully supervised instance segmentation model. 
To generate the pseudo mask labels, images containing $k$ instances are cropped around the corresponding extreme point annotations. These $k$ cropped images are then fed into the trained pseudo labeler, yielding a pseudo mask for each extreme point annotation. 
The decoupled design of the instance segmentation and pseudo labeling models allows for our pseudo labels to be seamlessly integrated into any fully supervised instance segmentation model.
% \hsh{\subsection{Learning a fully supervised model}
% \label{sec:subsection3_1}
% In the second stage, EXITS employs the trained \LHJ{pseudo label} generator to create pseudo mask labels, which are then used to train a fully supervised instance segmentation model.
% To generate pseudo mask labels, images containing multiple objects are cropped around each object to match the input format of the pseudo label generator. This process results in the generation of object-wise pseudo mask labels.
% Subsequently, these object-wise masks are combined according to the cropped regions to form the final pseudo mask labels.
% These pseudo mask labels can be applied to train any instance segmentation framework. 
% In our study, we apply SOLOv2~\cite{wang2020solov2} and Mask2Former~\cite{cheng2022masked} to demonstrate the generality and effectiveness of our approach.}


%Typically, in a fully supervised instance segmentation setting, a set of annotated training data is required, denoted as \( \mathcal{D} = \{ (X_n, C_n, B_n, M_n) \}_{n=1}^{N} \), where \( N \) is the number of images, \( C_n = \{c_n^k\}_{k=1}^{K} \), \( B_n = \{b_n^k\}_{k=1}^{K} \), and \( M_n = \{m_n^k\}_{k=1}^{K} \) denote the class-level, box-level, and pixel-level annotations, respectively, with \( K \) representing the number of instances in the image \( X_n \). 

% With given extreme point annotation \( E_n = \{e_n^k\}_{k=1}^{K} \), \( B_n \) can be obtained directly by reformatting $E_n$, and \( M_n \) is substituted by a pseudo mask \( \hat{M}_n \), generated by inputting the cropped region around the corresponding extreme point annotation into a pseudo labeler. Thanks to separated framework, our pseudo labels can be effortlessly incorporated into any fully supervised instance segmentation model, unlike other approaches~\cite{lan2021discobox,tian2021boxinst, li2022box,li2023sim, cheng2023boxteacher}.

%필요한 수식들 정리해놓기. 

==> sections/04_analysis_of_separated_case.tex <==

\section{Analysis of Separated Object}




\label{sec:analysis_of_separated_case}



==> sections/11_references.tex <==


z

==> supple/tables/tab_sup_mil_weight.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[ht]
\centering
\resizebox{0.5\linewidth}{!}{% Adjust the 0.8 to whatever suits your needs
\begin{tabular}{cccc}
\toprule
$\lambda_{mil}$ & AP & AP_{50} & AP_{75} \\
\midrule
2        & 39.7 & 67 & 40.1      \\ 
\rowcolor[HTML]{EFEFEF}10        & \textbf{40.4} & \textbf{67.4} & \textbf{41.4}      \\ 
20          & 39.8 & 66.7 & 40.4      \\ 
40          & 39.4 & 66.6 & 39.5      \\  \bottomrule
\end{tabular}%
}
\vspace{-2mm}
\caption{Effect of $\lambda_{mil}$ for the case of  $ | \hat{\mathcal{P}}_\text{FG} \cup \hat{\mathcal{P}}_\text{BG} | = 0 $.}
\label{tab:sup_mil_weight}
\vspace{-4mm}
\end{table}

==> supple/tables/tab_sup_point_and_crf_weight.tex <==


\begin{table}[ht]
\centering
\begin{minipage}[b]{0.45\linewidth} % Adjust the minipage width as needed
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
$\lambda_{point}$ & AP & AP_{50} & AP_{75} \\
\midrule
0.1        & 40.1 & 66.6 & 41.3      \\ 
\rowcolor[HTML]{EFEFEF}0.5        & \textbf{40.4} & \textbf{67.4} & \textbf{41.4}      \\ 
1          & 38.8 & 65.9 & 39.3      \\ 
2          & 38   & 66.2  & 38.1    \\ 
\bottomrule
\end{tabular}%
}
\caption{Effect of loss coefficient $\lambda_{point}$.}
\label{tab:sup_point_weight}
\end{minipage}
\hfill
\begin{minipage}[b]{0.425\linewidth} % Adjust the minipage width as needed
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
$\lambda_{crf}$ & AP & AP_{50} & AP_{75} \\
\midrule
0.1        & 37.9 & 65.9 & 37.6      \\ 
0.25        & 38.7 & 66.1 & 38.6      \\ 
\rowcolor[HTML]{EFEFEF}0.5          & \textbf{40.4} & \textbf{67.4} & \textbf{41.4}      \\ 
1          & 4   & 66.6  & 40.7    \\ 
\bottomrule
\end{tabular}%
}
\caption{Effect of loss coefficient $\lambda_{crf}$.}
\label{tab:sup_crf_weight}
\end{minipage}
\end{table}


==> supple/tables/tab_sup_tau.tex <==


\begin{table}[ht]
\centering
\begin{minipage}[b]{0.45\linewidth} % Adjust the minipage width as needed
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
$\tau_{\text{FG}}$ & AP & AP_{50} & AP_{75} \\
\midrule
0.00075        & 38.1 & 65.7 & 38.1      \\ 
\rowcolor[HTML]{EFEFEF}0.001        & 40.4 & 67.4 & 41.4      \\ 
0.00125          & 40.1   & 66.6  & 41.3    \\ 
0.0015          & \textbf{41.1} & \textbf{67.6} & \textbf{42.6}      \\ 
0.002          & 40.9   & 67.6  & 42.4    \\ 
\bottomrule
\end{tabular}%
}
\caption{Effect of $\tau_{\text{FG}}$}
\label{tab:sup_tau_fg}
\end{minipage}
\hfill
\begin{minipage}[b]{0.475\linewidth} % Adjust the minipage width as needed
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
$\tau_{\text{BG}}$& AP & AP_{50} & AP_{75} \\
\midrule
-0.00005        & 39.7 & 66.6 & 40.7      \\ 
\rowcolor[HTML]{EFEFEF}-0.0001        & \textbf{40.4} & \textbf{67.4} & \textbf{41.4}      \\ 
-0.00015         & 39.6 & 66.2 & 40.3      \\ 
-0.0002           & 38.8 & 65.9 & 39.1      \\ 
\bottomrule
\end{tabular}%
}
\caption{Effect of $\tau_{\text{BG}}$}
\label{tab:sup_tau_bg}
\end{minipage}
\end{table}


==> tables/tab_abl_component.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
 $\mathcal{P}_{\textrm{FG}} \cup \mathcal{P}_{\textrm{BG}}$ & $\hat{\mathcal{P}}_{\textrm{FG}} \cup {\hat{\mathcal{P}}_{\textrm{BG}}}$ & Point dropout & AP & AP_{50} & AP_{75} \\ \midrule \midrule
\xmark                 & \xmark     & \xmark                  & 37.6 & 64.8 & 37.9      \\ 
\cmark                 & \xmark     & \xmark                 & 38.0 & 65.3 & 38.6      \\
\cmark                 & \cmark     & \xmark                 & 39.8 & 67.1 & 40.4      \\
\cmark                 & \cmark     & \cmark                 & \textbf{40.4} & \textbf{67.4} & \textbf{41.4}       \\\bottomrule
\end{tabular}%
}
\caption{Ablation study of each component in $\mathcal{L}_{\text{point}}$.}
\label{tab:component}
\end{table}

==> tables/tab_abl_separatedcoco_wo_ref.tex <==
\begin{table}[]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcc}
\toprule
             & COCO (mIoU)         & Separated COCO (mIoU)         \\ \midrule \midrule
MAL         & 79.1                 & 59.3                    \\
\rowcolor[HTML]{EFEFEF} 
EXITS (Ours) & \textbf{79.4}              & \textbf{66.6}                    \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Pseudo label quality of the first stage.}
\vspace{-3mm}
\label{tab:sepcoco}
\end{table}

==> tables/tab_comp_sota_coco_v1.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{3pt}
    \begin{tabular}{lccccccccc}
    \toprule
    Method & InstSeg Backbone & InstSeg Model & ~~~~Sup~~~~ & $(\%)\text{Mask AP}_\text{val}$ & $(\%)\text{Mask AP}_\text{test}$ & $~~(\%)\text{Ret.}_\text{val}~~$ & $~~(\%)\text{Ret.}_\text{test}~~$ \\
    \midrule
    
    Mask R-CNN$^*$~\cite{mask_rcnn}       & ResNet-101                           & Mask R-CNN & Mask    & 38.6 & 38.8 & - & - \\
    Mask R-CNN$^*$~\cite{mask_rcnn}       & ResNeXt-101                          & Mask R-CNN & Mask    & 39.5 & 39.9 & - & - \\
    
    CondInst~\cite{tian2020conditional}   & ResNet-101                           & CondInst & Mask      & 38.6 & 39.1 & - & - \\
    SOLOv2~\cite{wang2020solov2}          & ResNet-50                            & SOLOv2 & Mask        & 37.5 & 38.4 & - & - \\
    SOLOv2~\cite{wang2020solov2}          & ResNet-101                           & SOLOv2 & Mask        & 37.8 & 39.7  & - & - \\
    SOLOv2~\cite{wang2020solov2}          & ResNet-101-DCN                       & SOLOv2 & Mask        &  41.7 & 41.8  & - & - \\
    SOLOv2~\cite{wang2020solov2}          & ResNeXt-101-DCN                       & SOLOv2 & Mask        &  42.4 & 42.7  & - & - \\
    Mask2Former~\cite{cheng2022masked}    & Swin-Small                           & Mask2Former & Mask   & \textbf{46.1} & \textbf{47.0} & - & - \\
    \midrule
    BBTP$\dagger$~\cite{hsu2019weakly}    & ResNet-101                           & Mask R-CNN  & Box    & - & 21.1 & - & 59.1 \\
    BoxInst~\cite{tian2021boxinst}        & ResNet-101                           & CondInst & Box       & 33.0 & 33.2 & 85.5 & 84.9 \\
    BoxLevelSet~\cite{li2022box}          & ResNet-101-DCN                       & SOLOv2 & Box         & 35.0 & 35.4 & 83.9 & 83.5\\
    DiscoBox~\cite{lan2021discobox}       & ResNet-50                            & SOLOv2 & Box         & 30.7 & 32.0 & 81.9 & 83.3 \\
    DiscoBox~\cite{lan2021discobox}       & ResNet-101-DCN                       & SOLOv2 & Box         & 35.3 & 35.8 & 84.7 & 85.9\\
    DiscoBox~\cite{lan2021discobox}       & ResNeXt-101-DCN                      & SOLOv2 & Box         & 37.3 & 37.9 & 88.0 & 88.8 \\
    BoxTeacher~\cite{cheng2023boxteacher} & ResNet-101                       & CondInst & Box         & - & 36.5 & - & - \\
    BoxTeacher~\cite{cheng2023boxteacher} & ResNet-101-DCN                       & CondInst & Box         & - & 37.6 & - & - \\
    BoxTeacher~\cite{cheng2023boxteacher} & Swin-Base                            & CondInst & Box       & - & 40.0 & - & - \\
    SIM ~\cite{li2023sim}                 & ResNet-101                             & CondInst & Box     & - & 35.3 & - & - \\
    SIM ~\cite{li2023sim}                 & ResNet-101-DCN-Bi-FPN                & CondInst & Box     & - & 37.4 & - & - \\
    BoxSnake ~\cite{Yang_2023_ICCV}       & ResNet-101-DCN-Bi-FPN                & CondInst & Box     & - & 37.4 & - & - \\
    \midrule
    Mask Auto-Labeler~\cite{lan2023vision} & ResNet-50 & SOLOv2 & Box                                    & 35.0 & 35.7 & 93.3 & 93.0 \\
    Mask Auto-Labeler~\cite{lan2023vision} & ResNet-101-DCN & SOLOv2 & Box                               & 38.2 & 38.7 & 91.6 & 92.6 \\
    Mask Auto-Labeler~\cite{lan2023vision} & ResNeXt-101-DCN & SOLOv2 & Box                              & 38.9 & 39.1 & 91.7 & 91.6 \\
    Mask Auto-Labeler~\cite{lan2023vision} & Swin-Small~\cite{liu2021swin} & Mask2Former~\cite{cheng2022masked} & Box & 43.3 & 44.1 & 93.9 & 93.8 \\
    \midrule
    Ours & ResNet-50 & SOLOv2 & Extreme Points                                                                                    & 36.1 (+1.1) & 36.9 (+1.2) & 96.3 (+3.0) & 96.1 (+3.1) \\
    Ours & ResNet-101-DCN & SOLOv2 & Extreme Points                                                                               & 00.0 & 00.0 & 00.0 & 00.0 \\
    Ours & ResNeXt-101-DCN & SOLOv2 & Extreme Points                                                                              & 40.5 (+1.6) & 40.9 (+1.8) & 95.5 (+3.8) & 95.8 (+4.2) \\
    Ours & Swin-Small~\cite{liu2021swin} & Mask2Former~\cite{cheng2022masked} & Extreme Points                                    & 44.2 (+0.9) & 45.0 (+0.9) & 95.9 (+2.0) & 95.7 (+1.9) \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{
    % Main results on COCO. Ret means the retention rate of $\frac{\text{box-supervised mask AP}}{\text{supervised mask AP}}$. MAL with SOLOv2/ResNeXt-101 outperforms DiscoBox with SOLOv2/ResNeXt-101 by 1.6\% on val2017 and 1.3\% on test-dev. Our best model (Mask2former/Swin-Small) achieves 43.3\% AP on val and 44.1\% AP on test-dev.
    Blah
    }
    \label{tab:coco_exp}
    \vspace{-1em}
    \end{table*}

==> tables/tab_comp_sota_coco_v2.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{3pt}
    \begin{tabular}{llccccc}
    \toprule
    Method &
    Backbone &
    ~~~~Sup~~~~ &
    $(\%)\text{Mask AP}_\text{val}$ &
    $(\%)\text{Mask AP}_\text{test}$ &
    $~~(\%)\text{Ret.}_\text{val}~~$ &
    $~~(\%)\text{Ret.}_\text{test}~~$ \\ \midrule \midrule
    SOLOv2~\cite{wang2020solov2}           & ResNet-50             & Mask           & 37.5          & 38.4          & -           & -           \\
    CondInst~\cite{wang2020solov2}         & ResNet-50             & Mask           & -             & 37.7          & -           & -           \\
    DiscoBox~\cite{lan2021discobox}        & ResNet-50             & Box            & 30.7          & 32.0          & 81.9        & 83.3        \\
    BoxTeacehr~\cite{cheng2023boxteacher}  & ResNet-50             & Box            & -             & 35.0          & -           & 92.8        \\
    Mask Auto-Labeler~\cite{lan2023vision} & ResNet-50             & Box            & 35.0          & 35.7          & 93.3        & 93.0        \\
    Ours                                   & ResNet-50             & Extreme Points & 36.1 (+1.1)   & 36.9 (+1.2)   & 96.3 (+3.0) & 96.1 (+3.1) \\ \midrule
    Mask R-CNN$^*$~\cite{mask_rcnn}        & ResNet-101            & Mask           & 38.6          & 38.8          & -           & -           \\
    CondInst~\cite{tian2020conditional}    & ResNet-101            & Mask           & 38.6          & 39.1          & -           & -           \\
    BBTP$\dagger$~\cite{hsu2019weakly}     & ResNet-101            & Box            & -             & 21.1          & -           & 59.1        \\
    BoxInst~\cite{tian2021boxinst}         & ResNet-101            & Box            & 33.0          & 33.2          & 85.5        & 84.9        \\
    BoxTeacher~\cite{cheng2023boxteacher}  & ResNet-101            & Box            & -             & 36.5          & -           & -           \\
    Ours                                   & ResNet-101            & Extreme Points & 00.0          & 00.0          & 00.0        & 00.0        \\ \midrule
    SOLOv2~\cite{wang2020solov2}           & ResNet-101-DCN        & Mask           & 41.7          & 41.8          & -           & -           \\
    BoxLevelSet~\cite{li2022box}           & ResNet-101-DCN        & Box            & 35.0          & 35.4          & 83.9        & 83.5        \\
    DiscoBox~\cite{lan2021discobox}        & ResNet-101-DCN        & Box            & 35.3          & 35.8          & 84.7        & 85.9        \\
    BoxTeacher~\cite{cheng2023boxteacher}  & ResNet-101-DCN        & Box            & -             & 37.6          & -           & -           \\
    SIM ~\cite{li2023sim}                  & ResNet-101-DCN-Bi-FPN & Box            & -             & 37.4          & -           & -           \\
    BoxSnake ~\cite{Yang_2023_ICCV}        & ResNet-101-DCN-Bi-FPN & Box            & -             & 37.4          & -           & -           \\
    Mask Auto-Labeler~\cite{lan2023vision} & ResNet-101-DCN        & Box            & 38.2          & 38.7          & 91.6        & 92.6        \\
    Ours                                   & ResNet-101-DCN        & Extreme Points & 00.0          & 00.0          & 00.0        & 00.0        \\ \midrule
    SOLOv2~\cite{wang2020solov2}           & ResNeXt-101-DCN       & Mask           & 42.4          & 42.7          & -           & -           \\
    DiscoBox~\cite{lan2021discobox}        & ResNeXt-101-DCN       & Box            & 37.3          & 37.9          & 88.0        & 88.8        \\
    Mask Auto-Labeler~\cite{lan2023vision} & ResNeXt-101-DCN       & Box            & 38.9          & 39.1          & 91.7        & 91.6        \\
    Ours                                   & ResNeXt-101-DCN       & Extreme Points & 40.5 (+1.6)   & 40.9 (+1.8)   & 95.5 (+3.8) & 95.8 (+4.2) \\ \midrule
    Mask2Former~\cite{cheng2022masked}     & Swin-Small~\cite{liu2021swin}            & Mask           & 46.1 & 47.0 & -           & -           \\
    Mask Auto-Labeler~\cite{lan2023vision} &
    Swin-Small~\cite{liu2021swin} &
    Box &
    43.3 &
    44.1 &
    93.9 &
    93.8 \\
    Ours &
      Swin-Small~\cite{liu2021swin} &
      Extreme Points &
      44.2 (+0.9) &
      45.0 (+0.9) &
      95.9 (+2.0) &
      95.7 (+1.9) \\ \bottomrule
    \end{tabular}%
    }
    \caption{}
    \label{tab:my-table}
\end{table*}

==> tables/tab_comp_sota_coco_v3.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{3pt}
        \begin{tabular}{llcccccc}
        \toprule
        Method &
          Backbone &
          ~~~~Sup~~~~ &
          InstSeg Model &
          $(\%)\text{Mask AP}_\text{val}$ &
          $(\%)\text{Mask AP}_\text{test}$ &
          $~~(\%)\text{Ret.}_\text{val}~~$ &
          $~~(\%)\text{Ret.}_\text{test}~~$ \\ \midrule \midrule
        SOLOv2~\cite{wang2020solov2}            & ResNet-50             & M         & SOLOv2         & 37.5 & 38.4 & -    & -    \\
        CondInst~\cite{wang2020solov2}          & ResNet-50             & M         & CondInst       & -    & 37.7 & -    & -    \\
        BoundaryFormer~\cite{Lazarow_2022_CVPR} & ResNet-50             & M         & BoundaryFormer & -    & 36.4 & -    & -    \\
        DiscoBox~\cite{lan2021discobox}         & ResNet-50             & B         & SOLOv2         & 30.7 & 32.0 & 81.9 & 83.3 \\
        BoxTeacher~\cite{cheng2023boxteacher}   & ResNet-50             & B         & CondInst       & -    & 35.0 & -    & 92.8 \\
        BoxSnake ~\cite{Yang_2023_ICCV}         & ResNet-50             & B         & BoundaryFormer & -    & 31.1 & -    & -    \\
        Mask Auto-Labeler~\cite{Lan_2023_CVPR}  & ResNet-50             & B         & SOLOv2         & 35.0 & 35.7 & 93.3 & 93.0 \\
        Ours &
          ResNet-50 &
          E         &
          SOLOv2 &
          \textbf{36.1 (+1.1)} &
          \textbf{36.9 (+1.2)} &
          \textbf{96.3 (+3.0)} &
          \textbf{96.1 (+3.1)} \\ \midrule
        Mask R-CNN$^*$~\cite{mask_rcnn}         & ResNet-101            & M         & Mask R-CNN     & 38.6 & 38.8 & -    & -    \\
        CondInst~\cite{tian2020conditional}     & ResNet-101            & M         & CondInst       & 38.6 & 39.1 & -    & -    \\
        BBTP$\dagger$~\cite{hsu2019weakly}      & ResNet-101            & B         & Mask R-CNN     & -    & 21.1 & -    & 59.1 \\
        BoxInst~\cite{tian2021boxinst}          & ResNet-101            & B         & CondInst       & 33.0 & 33.2 & 85.5 & 84.9 \\
        BoxTeacher~\cite{cheng2023boxteacher}   & ResNet-101            & B         & CondInst       & -    & 36.5 & -    & -    \\
        BoxSnake ~\cite{Yang_2023_ICCV}         & ResNet-101            & B         & BoundaryFormer & -    & 31.6 & -    & -    \\
        SIM~\cite{li2023sim}                   & ResNet-101            & B         & CondInst       & -    & 35.3 & -    & 90.3 \\
        Ours                                    & ResNet-101            & E         & SOLOv2         & 00.0 & 00.0 & 00.0 & 00.0 \\ \midrule
        SOLOv2~\cite{wang2020solov2}            & ResNet-101-DCN        & M         & SOLOv2         & 41.7 & 41.8 & -    & -    \\
        BoxLevelSet~\cite{li2022box}            & ResNet-101-DCN        & B         & SOLOv2         & 35.0 & 35.4 & 83.9 & 83.5 \\
        DiscoBox~\cite{lan2021discobox}         & ResNet-101-DCN        & B         & SOLOv2         & 35.3 & 35.8 & 84.7 & 85.9 \\
        BoxTeacher~\cite{cheng2023boxteacher}   & ResNet-101-DCN        & B         & CondInst       & -    & 37.6 & -    & -    \\
        SIM~\cite{li2023sim}                   & ResNet-101-DCN        & B         & CondInst       & -    & 37.4 & -    & -    \\
        Mask Auto-Labeler~\cite{Lan_2023_CVPR}  & ResNet-101-DCN        & B         & SOLOv2         & 38.2 & 38.7 & 91.6 & 92.6 \\
        Ours                                    & ResNet-101-DCN        & E         & SOLOv2         & 00.0 & 00.0 & 00.0 & 00.0 \\ \midrule
        SOLOv2~\cite{wang2020solov2}            & ResNeXt-101-DCN       & M         & SOLOv2         & 42.4 & 42.7 & -    & -    \\
        DiscoBox~\cite{lan2021discobox}         & ResNeXt-101-DCN       & B         & SOLOv2         & 37.3 & 37.9 & 88.0 & 88.8 \\
        Mask Auto-Labeler~\cite{Lan_2023_CVPR}  & ResNeXt-101-DCN       & B         & SOLOv2         & 38.9 & 39.1 & 91.7 & 91.6 \\
        Ours &
          ResNeXt-101-DCN &
          E         &
          SOLOv2 &
          \textbf{40.5 (+1.6)} &
          \textbf{40.9 (+1.8)} &
          \textbf{95.5 (+3.8)} &
          \textbf{95.8 (+4.2)} \\ \midrule
        Mask2Former~\cite{cheng2022masked} &
          Swin-Small~\cite{liu2021swin} &
          M &
          Mask2Former &
          46.1 &
          47.0 &
          - &
          - \\
        Mask Auto-Labeler~\cite{Lan_2023_CVPR} &
          Swin-Small~\cite{liu2021swin} &
          B &
          Mask2Former &
          43.3 &
          44.1 &
          93.9 &
          93.8 \\
        Ours &
          Swin-Small~\cite{liu2021swin} &
          E         &
          Mas2kFormer &
          \textbf{44.2 (+0.9)} &
          \textbf{45.0 (+0.9)} &
          \textbf{95.9 (+2.0)} &
          \textbf{95.7 (+1.9)} \\ \bottomrule
        \end{tabular}%
    }
    \caption{}
    \label{tab:my-table}
\end{table*}

% condinst: schedule 3x

==> tables/tab_comp_sota_coco_wo_ref.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{3pt}
\begin{tabular}{lcllcccc}
    \toprule
    Method &
      ~~~~Sup~~~~ &
      Backbone &
      InstSeg Model &
      \multicolumn{1}{l}{$\text{Mask AP}_\text{val}$} &
      \multicolumn{1}{l}{$\text{Mask AP}_\text{test}$} &
      \multicolumn{1}{l}{$~~(\%)\text{Ret.}_\text{val}~~$} &
      \multicolumn{1}{l}{$~~(\%)\text{Ret.}_\text{test}~~$} \\ \midrule \midrule
    \multicolumn{8}{c}{\textit{fully-supervised methods}} \\ \midrule
    SOLOv2 &
      M &
      ResNet-50 &
      SOLOv2 &
      37.5 &
      38.4 &
      - &
      - \\
    CondInst &
      M &
      ResNet-50 &
      CondInst &
      - &
      37.7 &
      - &
      - \\
    FastInst &
      M &
      ResNet-50 &
      FastInst &
      - &
      38.6 &
      - &
      - \\
    SOLOv2 &
      M &
      ResNet-101-DCN &
      SOLOv2 &
      41.7 &
      41.8 &
      - &
      - \\
    SOLOv2 &
      M &
      ResNeXt-101-DCN &
      SOLOv2 &
      42.4 &
      42.7 &
      - &
      - \\
    Mask2Former &
      M &
      Swin-Small &
      Mask2Former &
      46.1 &
      47.0 &
      - &
      - \\  \midrule
    \multicolumn{8}{c}{\textit{weakly-supervised methods}} \\ \midrule
    DiscoBox &
      B &
      ResNet-50 &
      SOLOv2 &
      30.7 &
      32.0 &
      81.9 &
      83.3 \\
    BoxTeacher&
      B &
      ResNet-50 &
      CondInst &
      - &
      35.0 &
      - &
      92.8 \\
    MAL &
      B &
      ResNet-50 &
      SOLOv2 &
      35.0 &
      35.7 &
      93.3 &
      93.0 \\
    \rowcolor[HTML]{EFEFEF}
    EXITS (Ours) &
      E &
      ResNet-50 &
      SOLOv2 &
      \textbf{36.1} &
      \textbf{36.9} &
      \textbf{96.3} &
      \textbf{96.1} \\
    BoxInst &
      B &
      ResNet-101-DCN &
      CondInst &
      - &
      35.0 &
      - &
      - \\
    DiscoBox &
      B &
      ResNet-101-DCN &
      SOLOv2 &
      35.3 &
      35.8 &
      84.7 &
      85.9 \\
    BoxLevelSet &
      B &
      ResNet-101-DCN &
      SOLOv2 &
      35.0 &
      35.4 &
      83.9 &
      83.5 \\
    BoxTeacher &
      B &
      ResNet-101-DCN &
      CondInst &
      - &
      37.6 &
      - &
      - \\
    SIM &
      B &
      ResNet-101-DCN &
      CondInst &
      - &
      37.4 &
      - &
      - \\
    MAL &
      B &
      ResNet-101-DCN &
      SOLOv2 &
      38.2 &
      38.7 &
      91.6 &
      92.6 \\
    \rowcolor[HTML]{EFEFEF}
    EXITS (Ours) &
      E &
      ResNet-101-DCN &
      SOLOv2 &
      \textbf{39.8} &
      \textbf{40.2} &
      \textbf{95.4} &
      \textbf{96.2} \\
    DiscoBox &
      B &
      ResNeXt-101-DCN &
      SOLOv2 &
      37.3 &
      37.9 &
      88.0 &
      88.8 \\
    MAL &
      B &
      ResNeXt-101-DCN &
      SOLOv2 &
      38.9 &
      39.1 &
      91.7 &
      91.6 \\
    \rowcolor[HTML]{EFEFEF}
    EXITS (Ours) &
      E &
      ResNeXt-101-DCN &
      SOLOv2 &
      \textbf{40.5} &
      \textbf{40.9} &
      \textbf{95.5} &
      \textbf{95.8} \\
    MAL &
      B &
      Swin-Small &
      Mask2Former &
      43.3 &
      44.1 &
      93.9 &
      93.8 \\
    \rowcolor[HTML]{EFEFEF}
    EXITS (Ours) &
      E &
      Swin-Small &
      Mask2Former &
      \textbf{44.2} &
      \textbf{45.0} &
      \textbf{95.9} &
      \textbf{95.7} \\\bottomrule
    \end{tabular}%
    }
    \caption{Results on COCO \texttt{val2017} and \texttt{test-dev}. We report performance using Mask Average Precision (Mask AP) and Retention rate (Ret, \%).
                  Retention rate is the performance ratio compared to its fully supervised counterpart.
                  Each method is trained with the supervision of either a mask (M), bounding box (B), or extreme points (E).
                  Note that the annotation cost of the bounding box and extreme points are equal.}
    \label{tab:coco}
    \vspace{-3mm}
\end{table*}

% condinst: schedule 3x

==> tables/tab_comp_sota_lvis_v1.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \addtolength{\tabcolsep}{7pt}
    \begin{tabular}{lccccccc}
    \toprule
    Method &  InstSeg Backbone & InstSeg Model & Training Data & Sup & $(\%)\text{Mask AP}_\text{val}$ & $(\%)\text{Ret.}_\text{val}$ \\
    \midrule
    Mask R-CNN~\cite{mask_rcnn} & ResNet-50-DCN & Mask R-CNN~\cite{mask_rcnn} & - & Mask & 21.7 & - \\
    Mask R-CNN~\cite{mask_rcnn} & ResNet-101-DCN & Mask R-CNN~\cite{mask_rcnn} & - & Mask & 23.6 & - \\
    Mask R-CNN~\cite{mask_rcnn} & ResNeXt-101-32x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & - & Mask & 25.5 & - \\
    Mask R-CNN~\cite{mask_rcnn} & ResNeXt-101-64x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & - & Mask & 25.8 & - \\
    \midrule
    Mask Auto-Labeler & ResNet-50-DCN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Box & 20.7 & 95.4 \\
    Mask Auto-Labeler & ResNet-101-DCN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Box & 23.0 & \textbf{97.4} \\
    Mask Auto-Labeler & ResNeXt-101-32x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Box & 23.7 & 92.9 \\
    Mask Auto-Labeler & ResNeXt-101-64x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Box & \textbf{24.5} & 95.0 \\
    \midrule
    Ours & ResNet-50-DCN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Extrene Points & 00.0 & 00.0 \\
    Ours & ResNet-101-DCN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Extrene Points & 00.0 & 00.0 \\
    Ours & ResNeXt-101-32x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Extrene Points & 00.0 & 00.0 \\
    Ours & ResNeXt-101-64x4d-FPN & Mask R-CNN~\cite{mask_rcnn} & LVIS v1 & Extrene Points & 00.0 & 00.0 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1em}
    \caption{LVIS.}
    \label{tab:lvis_exp}
    \vspace{-0.5em}
\end{table*}

==> tables/tab_comp_sota_voc.tex <==
\begin{table}
    \vspace{-3pt}
    \centering
    \renewcommand{\tabcolsep}{3pt}
    \renewcommand\arraystretch{1.1}
    % \scalebox{1.0}{
    \small
    \begin{tabular}{llccccc}
    \toprule
    Method & Backbone & AP & AP_{25} & AP_{50} & AP_{70} & AP_{75} \\
    \midrule \midrule
    BoxInst~\cite{tian2021boxinst} & R50 & 34.3 & - & 59.1 & - & 34.2 \\
    DiscoBox~\cite{lan2021discobox} & R50 & - & 71.4 & 59.8 & 41.7 & 35.5 \\
    BoxLevelSet~\cite{li2022box} & R50 & 36.3 & 76.3 & 64.2 & 43.9 & 35.9\\
    SIM~\cite{li2023sim} & R50 & 36.7 & - & 65.5 & - & 35.6 \\
    BoxTeacher~\cite{cheng2023boxteacher} & R50 & 38.6 & 77.6 & 66.4 & 46.1 & 38.7 \\
    MAL$\dagger$~\cite{Lan_2023_CVPR} & R50 & 37.6 & - & 64.8 & - & 37.9 \\
    MAL$\dagger$~\cite{Lan_2023_CVPR} & R50 & 37.6 & - & 64.8 & - & 37.9 \\
    \rowcolor[HTML]{EFEFEF} 
    Ours & R50 & \textbf{40.4} & 00.0 & \textbf{67.4} & 00.0 & \textbf{41.4} \\
    \midrule
    BBTP~\cite{hsu2019weakly} & R101 & - & 75.0 & 58.9 & 30.4 & 21.6 \\ 
    Arun \etal~\cite{arun2020weakly} & R101 & - & 73.1 & 57.7 & 33.5 & 31.2 \\   
    BBAM~\cite{lee2021bbam} & R101 & - & 76.8 & 63.7 & 39.5 & 31.8 \\
    BoxInst~\cite{tian2021boxinst} & R101 & 36.4 & - & 61.4 & - & 37.0 \\
    DiscoBox~\cite{lan2021discobox} & R101 & - & 72.8 & 62.2 & 45.5 & 37.5 \\
    BoxLevelSet~\cite{li2022box} & R101 & 38.3 & 77.9 & 66.3 & 46.4 & 38.7\\
    SIM~\cite{li2023sim} & R101 & 38.6 & - & 67.1 & - & 38.3 \\
    BoxTeacher~\cite{cheng2023boxteacher} & R101 & 40.3 & 78.4 & \textbf{67.8} & 48.0 & 41.3 \\
    MAL$\dagger$~\cite{Lan_2023_CVPR} & R101 & 37.4 & - & 65.7 & - & 39.1  \\
    \rowcolor[HTML]{EFEFEF} 
    Ours & R101 & \textbf{41.4} & 00.0 & 67.7 & 00.0 & \textbf{42.5} \\
    \bottomrule
    \end{tabular}
    \caption{PASCAL VOC.}
    \label{tab:voc_version1}
\end{table}
